Reasonable Space for the ${\lambda}$-Calculus, Logarithmically

Can the $\lambda$-calculus be considered a reasonable computational model? Can we use it for measuring the time $\textit{and}$ space consumption of algorithms? While the literature contains positive answers about time, much less is known about space. This paper presents a new reasonable space cost model for the $\lambda$-calculus, based on a variant over the Krivine abstract machine. For the first time, this cost model is able to accommodate logarithmic space. Moreover, we study the time behavior of our machine and show how to transport our results to the call-by-value $\lambda$-calculus.

==> 09-Related_Work.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Related Work}
The problem of giving time cost models for lambda-calculus which are reasonable is quite 
natural, and has been given partial answers since the 1990s. This investigation culminated 
with the first invariance result for  head-reduction, due to Accattoli and Dal Lago. This 
result was then generalized to other notions of reduction by Accattoli and his co-authors. 
In almost all these cases, the cost model under consideration is just the number of fired 
beta-redexes. Ralated to that, the problem of giving time efficient implementations of the 
lambda-calculus has been the object of many investigations. In this sense, it is certainly 
worth mentioning Levy's optimal evaluation, which however gives rise to a cost model which 
turns out to be provably not reasonable. (Magari dire che la riduzione ottimale nel caso 
weak è invece più "ragionevole".)

When space takes the place of time, literature becomes much sparser. 
Measuring the space consumption of functional programs is notoriously a nontrivial problem. 
This is due to the way functional programs are evaluated, i.e. through extensive use of 
sharing, which on the one hand permits to avoid duplication whenever possible, but on the 
other hand renders space essentially unaccountable. Remarkably, this is true also for pure 
functional programs, since environments and stacks are necessary even in the absence of 
references. The only invariance result related explicitly to space is the recent one by 
Forster et al: they prove that a cost model for space is linked to that of ordinary Turing 
Machines by a linear relationship with an additive overhead. As already mentioned, the cost 
model of Forster et al. can give rise to space costs which are exponential in the 
underlying time, thus being arguably unnatural. Dal Lago and Schopp's work on 
sublinear-space computation via the geometry of interaction shows that some higher-order 
functional programs, namely those typable in a substructural system akin to Girard et al.'s 
Bounded Linear Logic, can be attributed a sublinear space cost via compilation to circuits. 
Extending the paradigm to the pure lambda-calculus has recently been observed very unlikely 
by Accattoli et al.

Defining an invariant cost model and devising space efficient implementation methodologies 
are, once again, related but distinct goals. 
For example, implementation mechanisms that allow sharing but avoid garbage collection have 
been studied extensively, but they are not designed to offer precise guarantees, but rather 
to be efficient in practice.
Krishnaswami and his co-authors observe that space leaks are indeed possible while 
evaluating functional programs, and that this happens as soon as time is intrinsically 
higher than space, e.g. in functional reactive programming. Their solution consists in 
restricting the class of programs through a type system, again a substructural one.

Investigations about the complexity properties of abstract machines, and in particular the 
Krivine's abstract machine... 


==> 99-cbv.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Proofs of Section~\ref{sect:cbv}} 
 
 \begin{proposition}
 	The $\SpKAM$ and the $\SpLAM$ are weakly bisimilar when executed on 
 	$\detLam$-terms. Moreover, also their space consumption is the same.
 \end{proposition}
 \begin{proof}
	 The transitions of the \SpKAM not dealing with applications 
	 are 
	 identical to the corresponding ones of the \SpLAM (if one ignores the 
	 dump, 
	 that 
	 remains untouched). For the two transitions of the \SpKAM dealing with 
	 applications, we show that, when the argument is a variable or an 
	 abstraction 
	 (as in $\detLam$), the \SpLAM behaves as the \SpKAM. If the active term is 
	 $\tm\var$, indeed, the $\tokamseav$ transition of the \SpKAM is simulated 
	 on 
	 the \SpLAM by (with $\lenv(\var)=(\la\vartwo\tmtwo,\lenvtwo)$):
	\begin{center}$\begin{array}{lll}
	\splamstate{\stempty}{\tm\var}{\lenv}{\stack}&\tosplam& 
	\splamstate{\dentry{(\tm,\lenv|_\tm)}\stack}{\var}{\lenv|_\var}{\stempty}\\
	&\tosplam&\splamstate{\dentry{(\tm,\lenv|_\tm)}\stack}{\la\vartwo\tmtwo}{\lenvtwo}{\stempty}\\
	&\tosplam&\splamstate{\stempty}{\tm}{\lenv|_\tm}{(\la\vartwo\tmtwo,\lenvtwo)\cons\stack}\\
	&=&\splamstate{\stempty}{\tm}{\lenv|_\tm}{\lenv(\var)\cons\stack}
	\end{array}$\end{center}
	If the active term instead is 
	$\tm(\la\var\tmtwo)$, the $\tokamseanv$ transition of the \SpKAM is 
	simulated 
	on the \SpLAM by:
	\begin{center}$\begin{array}{lll}
		\splamstate{\stempty}{\tm(\la\var\tmtwo)}{\lenv}{\stack}&\tosplam& 
	\splamstate{\dentry{(\tm,\lenv|_\tm)}\stack}{\la\var\tmtwo}{\lenv|_{\la\var\tmtwo}}{\stempty}\\
	&\tosplam&\splamstate{\stempty}{\tm}{\lenv|_\tm}{(\la\var\tmtwo,\lenv|_{\la\var\tmtwo})\cdot\stack}\\
	\end{array}$\end{center}
	In particular, these macro steps show that to evaluate TM there is no need 
	of 
	the dump.
	Now, by defining a relation $\rel$ between states of the \SpKAM and the 
	\SpLAM 
	as
	\begin{center}$
	\state_K\,\rel\,\state_L\qquad\text{ iff }\qquad 
	\state_K=\spkamstate{\tm}{\lenv}{\stack}\text{ and } 
	\state_L=\splamstate{\stempty}{\tm}{\lenv}{\stack}
	$\end{center}
	the previous reasoning shows that $\rel$ is 
	a weak bisimulation preserving time and space complexity (modulo a constant 
	overhead).
\end{proof}

==> 99-encoding.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Encoding Space Sensitive TMs into the $\l$-Calculus}
\label{app:encoding}
\subsection{Preliminaries}

\paragraph{Deterministic $\l$-Calculus.}
The language and the evaluation contexts of the deterministic $\l$-calculus $\detLam$ are given by:
\begin{center}
	$\begin{array}{r@{\hspace{.5cm}}rlllllll}
	\mbox{Terms} & \tm,\tmtwo,\tmthree,\tmfour &\grameq& \val \mid  \tm \val\\
	\mbox{Values} & \val, \valtwo, \valthree & \grameq & \la\var\tm \mid \var\\\\
	\mbox{Evaluation Contexts} & \evctx  & \grameq & \ctxhole\mid  \evctx\val
	\end{array}$
\end{center}

Note that 
\begin{itemize}
	\item \emph{Arguments are values}: the right subterm of an application has to be a value, in contrast to what happens in the ordinary $\l$-calculus. 
	\item \emph{Weak evaluation}: evaluation contexts are \emph{weak}, \ie they do not enter inside abstractions. 
\end{itemize}

Evaluation is then defined by:
\begin{center}
	$\begin{array}{c@{\hspace{.5cm}}rll}
	\textsc{Rule at top level} & \multicolumn{3}{c}{\textsc{Contextual closure}} \\
	\!(\la\var\tm)\tmtwo \rtob \tm \isub\var\tmtwo &
	\multicolumn{3}{c}{\evctxp \tm \tobdet \evctxp \tmtwo \textrm{~~~if } \tm \rtob \tmtwo} \\
	\end{array}$
\end{center}

\emph{Convention}: to improve readability we omit some parenthesis, giving precedence to application with respect to abstraction. Therefore $\la \var \tm \tmtwo$ stands for $\la \var (\tm \tmtwo)$ and not for $(\la \var \tm) \tmtwo$, that instead requires parenthesis.

The name of this calculus is motivated by the following immediate lemma.

\begin{lemma}
	Let $\tm \in \detLam$. There is at most one $\tmtwo \in \detLam$ such that $\tm \tob \tmtwo$, and in that case $\tm$ is an application.
\end{lemma}

\begin{proof}
	By induction on $\tm$. If $\tm$ is a value then it does not reduce. Then assume that $\tm$ is an application $\tm = \tmtwo \val$. Let's apply the \ih to $\tmtwo$. Two cases:
	\begin{enumerate}
		\item \emph{$\tmtwo$ reduces and it is an application}: then $\tm$ has one redex, the one given by $\tmtwo$ (because $\ctxhole \val$ is an evaluation context), and no other one, because $\val$ does not reduce and $\tmtwo$ is not an abstraction by the \ih
		
		\item \emph{$\tmtwo$ does not reduce}: if $\tmtwo$ is not an abstraction then $\tm$ is normal, otherwise $\tmtwo = \la\var\tmthree$ and $\tm = (\la\var\tmthree) \val$ has exactly one redex.
	\end{enumerate}
\end{proof}

\paragraph{Fixpoint.} Let $\fix$ be the term $\theta\theta$, where
$$
\theta \defeq \la\var \la\vartwo \vartwo(\la\varthree \var \var \vartwo 
\varthree).
$$
Now, given a term $\tmtwo$ let us show that $\fix\tmtwo$ is a fixpoint of 
$\tmtwo$ up to $\eta$-equivalence.
$$\begin{array}{lcllll}
	\fix\tmtwo  
	& = &
	(\la\var \la\vartwo \vartwo(\la\varthree \var \var \vartwo \varthree)) 
	\theta 
	\tmtwo \\
	& \tobdet & 
	(\la\vartwo \vartwo(\la\varthree \theta \theta \vartwo \varthree)) \tmtwo \\
	
	& \tobdet & 
	\tmtwo (\la\varthree \theta \theta \tmtwo \varthree)\\ 
	& = &
	\tmtwo (\la\varthree \fix \tmtwo \varthree)\\
	& =_\eta &
	\tmtwo (\fix \tmtwo)
\end{array}$$



\paragraph{Encoding alphabets.} Let $\alpone=\{\elone_1,\ldots,\elone_n\}$ be a 
finite alphabet. Elements of $\alpone$ are encoded
as follows:
$$
\cod{\elone_i}{\alpone} \defeq \lambda\var_1.\ldots.\lambda\var_n.\var_i \;.
$$
When the alphabet will be clear from the context we will simply write 
$\cods\elone_i$. Note that 
\begin{enumerate}
	\item the representation fixes a total order
	on $\alpone$ such that $\elem_i\leq \elem_j$ iff $i\leq j$;
	\item the representation of an element $\cod{\elone_i}{\alpone}$ requires 
	space linear (and not logarithmic) in $\size\alpone$. But, since $\alpone$ 
	is fixed, it actually requires constant space.
\end{enumerate}

\paragraph{Encoding strings.} A string in
$\strone\in\alpone^*$ is represented by a term
$\encp\strone{\alpone^*}$, defined by induction on the structure of $\strone$ 
as follows:
\begin{align*}
	\enc{\varepsilon}^{\alpone^*} & \defeq 
	\lambda\var_1.\ldots.\lambda\var_n.\lambda\vartwo.\vartwo\;,\\
	\enc{\elone_i\strtwo}^{\alpone^*} & \defeq \lambda\var_1.\ldots.
	\lambda\var_n.\lambda\vartwo.\var_i\enc{\strtwo}^{\alpone^*}.
\end{align*}
Note that the representation depends on the cardinality
of $\alpone$. In other words, if $\strone\in\alpone^*$
and $\alpone\subset\alptwo$, 
$\enc\strone^{\alpone^*}\neq\enc\strone^{\alptwo^*}$. In particular, 
$\size{\enc\strone^{\alpone^*}} = \Theta(\size\strone\cdot\size\alpone)$. The 
size of the alphabet is however considered as a fixed parameter, and so we 
rather have $\size{\enc\strone^{\alpone^*}} = \Theta(\size\strone)$.

\begin{lemma}[Appending a character in constant time]
	\label{l:append-char}
	Let $\alpone$ be an alphabet and $\elem \in\alpone$ one of its characters. 
	There is 
	a term $\appendalpchar\alpone\elem$ 
	such that for every
	continuation $\cont$ and every string $\strone\in\alpone^*$, 
	$$
	\appendalpchar\alpone \elem \cont  \enc\strone
	\tobdet^{\bigo{1}} 
	\cont \enc{(\elem\strone)}.
	$$
\end{lemma}
\begin{proof}
	Define the term $\appendalpchar \alpone \elem \defeq \la{\cont'} 
	\la{\strone'} \cont'(\lambda \var_1.\ldots.\lambda 
	\var_{\size\alpone}.\lambda \vartwo.\var_{i_\elem} \strone')$ where 
	$i_\elem$ is the index of $\elem$ in 
	the ordering of $\alpone$ fixed by its encoding, that appends the character 
	$\elem$ to the string $\strone'$ relatively to the alphabet $\alpone$. We 
	have:
	$$\begin{array}{rclcl}
		\appendalpchar \alpone  \elem \cont \enc\strone
		& = &
		(\la{\cont'} \la{\strone'} \cont'(\lambda \var_1.\ldots.\lambda 
		\var_{\size\alpone}.\lambda \vartwo.\var_{i_\elem} \strone')) 
		\cont\enc\strone  \\
		& \tobdet^2 &
		\cont(\lambda \var_1.\ldots.\lambda \var_{\size\alpone}.\lambda 
		\vartwo.\var_{i_\elem}\enc{\strone}) \\
		& = &
		\cont \enc{(\elem \strone)}.
	\end{array}$$
	
	%The term that appends a generic character $\elem$ to a string $\strone$ is 
	%obtained by using the encoding of $\elem$ to select the right 
	%$\appendchar{\elem_i}$ to apply to the encoding of $\strone$. Define:
	%$$
	%\appendalph{\alpone} \defeq \lambda \cont.\lambda a.\lambda \strone.a 
	%\appendchar{\elem_1}\ldots \appendchar{\elem_{\size\alpone}}\strone \cont
	%$$
	%Then:
	%\begin{eqnarray*}
	%  \appendalph{\alpone} \cont \cods{\elem_i} \cods{\strone}
	%  & = &
	%  (\lambda \cont.\lambda a.\lambda \strone.a \appendchar{\elem_1}\ldots 
	%\appendchar{\elem_{\size\alpone}}\strone \cont) \cont \cods{\elem_i} 
	%\cods{\strone}\\
	%  & \tobdet^3 &
	%  \cods{\elem_i} \appendchar{\elem_1} \ldots 
	%\appendchar{\elem_{\size\alpone}} \cods{\strone} \cont\\
	%  & \tobdet^{\size\alpone} & 
	%  \appendchar{\elem_i} \cods{\strone}\cont\\
	%  & \tobdet^2 &
	%  \cont\cods{(\elem_i \strone)}.
	%\end{eqnarray*}
\end{proof}

\subsection{Binary Arithmetic}

In order to navigate the input word, we consider a counter (in binary). Moving 
the head left (respectively right) amounts to decrement (respectively 
increment) the counter by one. The starting idea is to see a number as its 
binary string representation and to use the Scott encoding of strings. Since it 
is tricky to define the successor and predecessor on such an encoding, we 
actually define an ad-hoc encoding.

The first unusual aspect of our encoding is that the binary string is 
represented in reverse order, so that the representation of $2$ is $01$ and not 
$10$. This is done to ease the definition of the successor and predecessor 
functions as $\l$-terms, which have to process strings from left to right, and 
that with the standard representation would have to go to the end of the string 
and then potentially back from right to left. With a reversed representation, 
these functions need to process the string only once from left to right.

The second unusual aspect is that, in order to avoid problems with strings made 
out of all $0$s and strings having many $0$s on the right (which are not 
meaningful), we collapse all suffixes made out of all $0$ on to the empty 
string. A consequence is that the number $0$ is then represented with the empty 
string. Non-rightmost $0$ bits are instead represented with the usual Scott 
encoding.

If $n\in\nat$ we write $\ntostr n$ for the binary string representing $n$. Then 
we have:

\[
\begin{array}{lll}
	\ntostr 0 &\defeq&\ems
	\\[3pt]
	\ntostr 1 &\defeq&1
	\\[3pt]
	\ntostr 2 &\defeq& 01
	\\[3pt]
	\ntostr 3 &\defeq& 11
	\\[3pt]
	\ntostr 4 &\defeq& 001
	\\
\end{array}
\]
And so on. Binary strings are then encoded as $\l$-terms using the Scott 
encoding, as follows:
\[
\begin{array}{lll}
	\enc{\ems}&\defeq&\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}
	\\[3pt]
	\enc{0\cons\str}&\defeq&\la{\var_0}{\la{\var_1}{\la\vartwo\var_0\enc{\str}}}
	\\[3pt]
	\enc{1\cons\str}&\defeq&\la{\var_0}{\la{\var_1}{\la\vartwo\var_1\enc{\str}}}
	\\
\end{array}
\]

\paragraph{Successor Function.} The successor function $\succf$ on the reversed 
binary representation can be defined as follows (in Haskell-like syntax):
\[
\begin{array}{llll}
	\succf &\ems& = &1\\
	\succf &0\cons\str& = &1\cons\str\\
	\succf &1\cons\str& = &0\cons(\succf\,\str)\\
\end{array}
\]

For which we have $\succf(\ntostr n) = \ntostr{n+1}$.

\begin{lemma}
	\label{l:succ}
	There is 
	a $\l$-term $\succl$ 
	such that for every
	continuation $\cont$ and every natural number $\counter\in\nat$, 
	$$
	\succl\, \cont  \enc{\ntostr\counter}
	\tobdet^{\bigo{\size{\ntostr\counter}}} 
	\cont\, \enc{\succf\, \ntostr\counter}.
	$$
\end{lemma}

\input{./proofs/preliminaries/succ-proof}

\paragraph{Predecessor Function.} We now define and implement a predecessor 
function. We define it assuming that it shall only be applied to the enconding 
$\ntostr n$ of a natural number $n$ different from $0$, as it shall indeed be 
the case in the following. Such a predecessor function $\predf$ is defined as 
follows on the reversed binary representation (in Haskell-like syntax):
\[
\begin{array}{lllll}
	\predf &0\cons\str& = &1\cons(\predf\,\str)\\
	\predf &1\cons\ems& = &\ems\\
	\predf &1\cons b\cons\str& = &0\cons b\cons\str\\
\end{array}
\]
It is easily seen that $\predf (\ntostr n) = \ntostr{n-1}$ for all 
$0<n\in\nat$. Note that $\predf(\ntostr n)$ does not introduce a rightmost $0$ 
bit when it changes the rightmost bit of $\ntostr n$, that is, $\predf\, 001 = 
11$ and not $110$.

\begin{lemma}
	\label{l:pred}
	There is a $\l$-term $\predl$ such that for every continuation $\cont$ and 
	every natural number $1\leq\counter\in\nat$, 
	$$
	\predl\, \cont  \enc{\ntostr\counter}
	\tobdet^{\bigo{\size{\ntostr\counter}}} 
	\cont\, \enc{\predf\, \ntostr\counter}.
	$$
\end{lemma}

\input{./proofs/preliminaries/pred-proof}


\paragraph{Lookup Function.} Given a natural number $\counter$, we need to be 
able to extract the $\counter+1$-th character from a non-empty string $\str$. 
The partial function $\lookupf$ can be defined as follows (in Haskell-like 
syntax):
\[
\begin{array}{llllll}
	%\lookupf &\str&\ems& = &0\\
	\lookupf &\ntostr 0&(c\cons\str)& = &c\\
	\lookupf &\ntostr n&(c\cons\str)& = &\lookupf\ (\predf\, \ntostr n)\ \str & 
	\mbox{if }n>0\\
\end{array}
\]

\begin{lemma}\label{l:look}
	There is a $\l$-term $\lookupl$ such that for every continuation $\cont$, 
	every natural number $n$ and every non-empty string $\inputstr\in\Bool^+$, 
	$$\lookupl\,k\enc{\ntostr n}\enc{\inputstr} \ \ \tobdet^{\bigo{n\log n}} \ 
	\ k\,\cods{\lookupf\, \ntostr n \inputstr}.$$
\end{lemma}

\input{./proofs/preliminaries/lookup-proof}

\subsection{Encoding Turing Machines}
\paragraph{Turing Machines.}
Let $\Boolin \defeq \set{0,1,\stsym,\ensym}$ and $\Boolb \defeq 
\set{0,1,\elemblank}$ where $\stsym$ and $\ensym$ delimit the input (binary) 
string, and  
$\elemblank$ is our notation for the blank symbol. 
A deterministic binary Turing machine $\mathcal{M}$ \emph{with input} is a 
tuple 
$(\States,\statein,\statefint,\statefinf,\delta)$ consisting of:
\begin{itemize}
	\item
	A finite set $Q=\{\state_1,\ldots,\state_m\}$ of \emph{states};
	\item
	A distinguished state $\statein\in Q$, called the \emph{initial
		state};
	\item
	Two distinguished states $\Statesfin\defeq\set{\statefint,\statefinf} 
	\subseteq \States$, 
	called the 
	\emph{final
		states}; 
	\item
	A partial \emph{transition function} 
	$\delta:\Boolin\times\Boolb\times\States\rightharpoonup 
	\{-1,+1,0\}\times\Boolb\times\{\leftarrow,\rightarrow,\downarrow\} \times 
	\States$
	such that
	$\delta(\bool,\elem,\state)$ is defined only if $\state\notin 
	\Statesfin$.
\end{itemize}
A configuration for $\mathcal{M}$ is a tuple
$$(\inputstr,\counter,\wstrl, \elem, \wstrr, \state) \in 
\Boolin^*\times\Nset\times\Boolb^*\times\Boolb\times\Boolb^*\times \States$$
where:
\begin{itemize}
	\item $\inputstr$ is the 
	immutable input string and is formed as 
	$\inputstr=\stsym\cons\str\cons\ensym,\ \str \in \Bool^*$;
	\item $\counter\in \Nset$ represents the position of the input head. It is 
	meant to be represented in binary (that is, as an element of $\Bool^*$), to 
	take space $\log \counter$, but for ease of reading we keep referring to it 
	as a number rather than as a string;
	\item $\wstrl \in \Boolb^*$ is the work tape on the left of the work head;
	\item $\elem \in \Boolb$ is the element on the cell of the work tape read 
	by the work 
	head;
	\item $\wstrr \in \Boolb^*$ is the work tape on the right of the work head;
	\item $\state \in \States$ is the state of the machine.
\end{itemize}
For readability, we usually write a configuration $(\inputstr,\counter,\wstrl, 
\elem, \wstrr, \state)$ as $(\inputstr,\counter \csep \wstrl, \elem , \wstrr 
\csep \state) $, separating the input components, the working components, and 
the current state.


Given an input string $\inputstr \in\Boolin^*$ (where 
$i=\stsym\cons\str\cons\ensym$ and $\str\in\Bool^*$) we define:
\begin{itemize}
	\item the \emph{initial configuration} $\initconfigs$
	for $\inputstr$ is $\initconfigs \defeq 
	(\inputstr,0 \csep \varepsilon,\elemblank,\varepsilon 
	\csep \statein)$,
	\item the \emph{final configuration}
	$\config_{\tt fin} \defeq 
	(\str,\counter \csep \wstrl,\elem,\wstrr \csep\state)$, where 
	$\state\in\Statesfin$.	
\end{itemize}
For readability, a transition, say, $\delta(\inputstr_{\counter},\elem,\state) 
= 
(-1,\elem',\leftarrow, \state')$, is usually written as $(-1 \csep 
\elem',\leftarrow \csep \state')$ to stress the three components corresponding 
to those of configurations (input, work, state).

As in Goldreich, we assume that the machine never scans the input beyond the 
boundaries of the input. This does not affects space complexity.

\emph{An example of transition}: if $\delta(\inputstr_{\counter},\elem,\state) 
= 
(-1 \csep \elem',\leftarrow \csep \state')$, then $\M$ 
evolves from $\config = (\inputstr,n \csep \wstrl\elem'',\elem,\wstrr \csep 
\state)$, 
where the $\counter$th character of $\inputstr$ is $\inputstr_{\counter}$, 
to 
$\configtwo = (\inputstr,n-1\csep \wstrl,\elem'',\elem'\wstrr \csep \state')$ 
and if 
the tape on the 
left of the work head is empty, \ie if $\config = 
(\inputstr,n \csep \varepsilon,\elem,\wstrr \csep \state)$, then the content of 
the 
new head cell 
is a blank symbol, that is, $\configtwo \defeq 
(\inputstr,n-1 \csep \varepsilon,\elemblank,\elem'\wstrr \csep \state')$. The 
same happens if the tape on the right of the work head is empty. If $\M$ has a 
transition 
from $\config$ to $\configtwo$ we write $\config \tomachtur \configtwo$. A 
configuration having as state a final state $\state\in\Statesfin$ is 
\emph{final} and cannot evolve.


A Turing machine $(\States,\statein,
\statefint,\statefinf,\delta)$ computes the function 
$f:\Bool^*\rightarrow\Bool$ 
in time $T:\Nset\rightarrow\Nset$ and space  $S:\Nset\rightarrow\Nset$
if for every $\istr\in\Bool^+$, the
initial configuration for $\istr$ evolves to a final configuration of state 
$\state_{f(\istr)}$ in $T(\size\istr)$ steps and using at most $S(\size\istr)$ 
cells on the work tape.

\paragraph{Encoding configurations.} A configuration 
$(\inputstr,\counter \csep \strone,\elem,\strtwo \csep\state)$ of a machine
$\M = (\States,\statein, \statefint,\statefinf,\delta)$ is 
represented by
the term
$$
\encp{(\inputstr,\counter \csep \wstrl,\elem,\wstrr \csep \state)}{\M}
\defeq
\lambda x. (x \encp{\inputstr}{\Bool^+}\encp{\ntostr \counter}{\Bool}\;
\encp{\wstrl^{\rop}}{\Boolb^*}\;\cod{\elem}{\Boolb}\;\encp{\wstrr}{\Boolb^*}\;\cod{\state}{\States}).
$$
where $\wstrl^{\rop}$ is the string $\wstrl$ with the elements in reverse 
order. 
We shall often rather write
$$
\enc{(\inputstr,\counter \csep \wstrl,\elem,\wstrr \csep \state)}
\defeq
\lambda x. (x\; \enc{\inputstr}\; \enc{\ntostr \counter}\;
\enc{\wstrl^{\rop}}\;\cods\elem \; \enc\wstrr \; \cods\state).
$$
letting the superscripts implicit. To ease the reading, we sometimes use the 
following  notation for tuples 
$\tuple{\tmfive,\tmsix \csep \tm,\tmtwo,\tmthree \csep \tmfour} \defeq 
\lambda x. (x \tmfive\tmsix\tm \tmtwo \tmthree \tmfour)$, so that 
$\enc{(\inputstr,\counter \csep \wstrl,\elem,\wstrr \csep \state)} = 
\tuple{\enc{\inputstr},\enc{\ntostr \counter} \csep \enc{\wstrl^{\rop}}, 
\cods\elem, 
	\enc\wstrr \csep \cods\state}$.

%Please note that the size of a configuration 
%$\enc\config=\enc{(\strone,\elem,\strtwo,\state)}$ is linear in 
%$\size\States$ and $\size{\strone\cons a\cons\strtwo}$.

\paragraph{Turning the input string into the initial configuration.} The 
following lemma provides the term $\inits $ that builds the initial 
configuration.

\begin{lemma}[Turning the input string into the initial configuration]
	\label{l:init-config}
	Let $\M=(\States,\statein,
	\statefint,\statefinf,\delta)$ be a Turing machine. There is a term 
	$\init\M{}$, or 
	simply $\inits$, such that for every input string $\inputstr\in\Boolin^*$ 
	(where 
	$i=\stsym\cons\str\cons\ensym$ and $\str\in\Bool^*$):
	$$\inits\, \cont\, \enc{\inputstr} \ \ \tobdet^{\Theta(1)} \ \
	\cont\, \enc\initconfigs$$ 
	where $\initconfigs$ is the initial configuration of $\M$ for $\inputstr$.
\end{lemma}

\input{proofs/TM-to-lambda/init-proof}

\paragraph{Extracting the output from the final configuration.}

\begin{lemma}[Extracting the output from the final configuration]
	\label{l:final-config}
	Let $\M=(\States,\statein,
	\statefint,\statefinf,\delta)$ be a Turing machine. There is 
	a term $\final\M{}$, or simply $\finals$, such that  for every final
	configuration 
	$\config$ of state $\state\in\Statesfin$
	
	\[\finals\, \cont\, \enc\config \tobdet^{\Theta(\size\States)} 
	\begin{cases}
		\cont(\la\var{\la\vartwo\var)}&\text{ if }\state= \statefint\\
		\cont(\la\var{\la\vartwo\vartwo)} &\text{ if }\state= \statefinf
	\end{cases}\]
\end{lemma}

\input{proofs/TM-to-lambda/final-proof}

\paragraph{Simulation of a machine transition.} Now we show how to encode the 
transition function $\delta$ of a Turing machine as a $\l$-term in such a way 
to simulate every single transition in constant? time. This is the heart of the 
encoding, and the most involved proof.

\begin{lemma}[Simulation of a machine transition]
	\label{l:trans-sim}
	Let $\M=(\States,\statein,\statefint,\statefinf,\delta)$ be a Turing 
	machine. There is a term 
	$\trans{\M}$, or 
	simply 
	$\transs$,
	such that for every configuration 
	$\config$ of input string $\istr\in\Bool^{+}$: 
	\begin{itemize}
		\item \emph{Final configuration}:
		if $\config$ is a final configuration
		then $\transs\, \cont\, 
		\enc\config \tobdet^{\bigo{\size\istr\log{\size\istr}}} \cont\, 
		\enc\config$;
		\item \emph{Non-final configuration}: if $\config \tomachtur 
		\configtwo$ then 
		$\transs\, \cont\, 
		\enc\config 
		\tobdet^{\bigo{\size\istr\log{\size\istr}}} \transs\, \cont\, 
		\enc\configtwo$.
	\end{itemize}
\end{lemma}

\begin{proof}
	\input{./proofs/TM-to-lambda/one-step-simulation-proof} 
\end{proof}

Straightforward inductions on the length of executions provide the following 
corollaries.

\begin{corollary}[Executions]
	\label{coro:exec}
	Let $\M$ be a Turing machine. Then there exist a term $\transs$ encoding 
	$\M$ 
	as given by \reflemma{trans-sim} such that
	for every configuration $\config$ of input string $\istr\in\Bool^{+}$
	\begin{enumerate}
		\item \emph{Finite computation}:
		if $\configtwo$ is a final configuration reachable from $\config$ in 
		$n$ 
		transition steps
		then there exists a derivation $\run$ such that $\run:\transs\, \cont 
		\cods\config \tobdet^{\bigo{(n+1)\size\istr\log{\size\istr}}} \cont 
		\cods\configtwo$;
		\item \emph{Diverging computation}: if there is
		no final configuration reachable from $\config$ then $\transs\, \cont 
		\cods\config$ diverges.
	\end{enumerate}
\end{corollary}

\paragraph{The simulation theorem.}
We now have all the ingredients for the final theorem of this note.

\begin{theorem}[Simulation]
	Let $f:\Bool^*\rightarrow\Bool$ a function computed by a Turing machine
	$\M$ in time $T_{\M}$. Then there is an encoding $\cods{\cdot}$ into 
	$\detLam$ of $\Bool$, strings, and Turing machines over $\Bool$ such that 
	for every $\istr\in\Bool^+$, there exists $\run$ such that
	$\run:\cods\M \cods\istr \tobdet^n \cods{f(\istr)}$
	where $n=\Theta((T_{\M}(\size\istr)+1)\cdot \size\istr\cdot 
	\log{\size\istr})$.
\end{theorem}

\begin{proof}
	Morally, the term is simply
	$$
	\enc\M \defeq \inits (\transs(\finals(\lambda w.w))
	$$
	where $\lambda w.w$ plays the role of the initial continuation.
	
	Such a term however does not belong to the deterministic $\l$-calculus, 
	because the right subterms of applications are not always values. The 
	solution is simple, it is enough to $\eta$-expand the arguments. Thus, 
	define
	
	$$
	\enc\M \defeq \inits (\la\vartwo\transs(\la \var\finals(\lambda 
	w.w)\var)\vartwo)
	$$
	
	
	Then
	$$\begin{array}{lll}
		\enc\M \cods{\istr} 
		& = & \\
		\inits (\la\vartwo\transs (\la \var\finals (\lambda w.w)\var)\vartwo) 
		\cods{\istr} 
		& \tobdet^{\Theta(1)} & (\mbox{by }\reflemmaeq{init-config})\\    
		(\la\vartwo\transs (\la \var\finals (\lambda w.w)\var)\vartwo) 
		\cods{\initconfig}
		& \tobdet\\
		\transs (\la \var\finals (\lambda w.w)\var) \cods{\initconfig}
		& \tobdet^{\Theta((T_{\M}(\size\istr)+1)\cdot \size\istr \cdot 
		\log{\size\istr})} & (\mbox{by }\refcoroeq{exec})\\
		(\la \var\finals (\lambda w.w)\var) \cods{\config_{\tt fin}(f(\istr))}
		& \tobdet\\
		\finals (\lambda w.w) \cods{\config_{\tt fin}(f(\istr))}
		& \tobdet^{\Theta(\size\States)} & (\mbox{by 
		}\reflemmaeq{final-config})\\    
		(\lambda w.w) \cods{f(\istr)}
		& \tobdet &\\
		\cods{f(\istr)}
	\end{array}$$
\end{proof}


==> 99-reasonability.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Proofs of Section~\ref{sect:reasonability}}
\label{app:reasonability}
The first part of this appendix is devoted to the proof of the main theorem of 
the paper, \ie the space reasonable simulation of TMs into the $\l$-calculus 
(better, the \SpKAM). It is a boring proof, where we simply execute the image 
of the encoding of TMs into the $\l$-calculus with the \SpKAM.

First, we need to understand how a TM configuration is represented in the 
\SpKAM, \ie how it is mapped to environments and closures.

\begin{definition}
A configuration $\config$ of a TM is represented as a KAM closure 
$\config^{\kop}$ in 
the 
following way:
\[
(\inputstr,\counter,\strone,\elem,\strtwo,\state)^{\kop}\defeq(\tuple{f,c,m,\cods\elem,
	d,\cods\state},\esub f{(\enc\inputstr,\stempty)},\esub c {n^{\kop}}, 
\esub m {\str{^{\kop}}}, \esub d {\strtwo^{\kop}})
\]
where
$\str^{\kop}=\begin{cases}
	(\cods\ems,\stempty) & \text{if }\str=\ems\\
	(\lambda \var_1.\ldots.\lambda \var_{\size\alpone}.\lambda 
	\vartwo.\var_{i_\elem}z,\esub z {r^{\kop}}) & \text{if 
	}\str=\elem_i\strtwo
\end{cases}
$
\end{definition}

We observe that this representation preserves the space consumption, \ie it is 
reasonable.
\begin{lemma}\label{l:config-size}
	Let $\config\defeq(\inputstr,\counter,\strone,\elem,\strtwo,\state)$ be a 
	configuration of a Turing machine and 
	$\size{\config}\defeq\size\strone+\size\strtwo$ its 
	space consumption. Then 
	$\size{\config^{\kop}}=\Theta(\size{\config}+\log(\size 
	i))$.
\end{lemma}
In this lemma, we have already considered that the size of pointers inside 
$\counter^\kop$, $\str^\kop$, $\strtwo^\kop$ is constant and that 
$n\leq\log\size\istr$.

Now we are able to prove the theorem. A series of intermediate lemmata, about 
the different combinators used in the encoding ($\inits,\finals,\transs$), are 
necessary. They are stated 
and proved below the main statement . By $\too^*_f$, we mean that the space 
consumption of that series of transitions is $f$.

\begin{theorem}[TM are simulated by the \SpKAM in reasonable space]
	There is an encoding $\enc{\cdot}$ of log-sensitive TM into 
	$\detLam$ such that if the run $\run$ of the TM $M$ on input 
	$\istr\in\Bool^{*}$:
	\begin{enumerate}
		\item 
		\emph{Termination}: ends in $\state_{\bool}$ with $\bool\in\Bool$, then
		there is a complete sequence $\runtwo:\enc M\, \enc\istr \tobdet^n 
		\enc{\bool}$
		where $n=\Theta((T_{\textrm{TM}}(\run)+1)\cdot \size\istr\cdot 
		\log{\size\istr})$.
		
		\item 
		\emph{Divergence}: diverges, then $\enc M\, \enc\istr$ is 
		$\tobdet$-divergent.
		
		\item 
		\emph{\SpKAM}: the space used by the \SpKAM to simulate the evaluation 
		of  point 1 is $\bigo{S_{\textrm{TM}}(\run) +\log\size\istr}$ if $\enc 
		M$ 
		and $\enc\istr$ have separate address spaces.
	\end{enumerate}
\end{theorem}
\begin{proof}
	The first two points are proved in the section devoted to the encoding of 
	TMs into the $\l$-calculus. We concentrate on the third point.
	
	We simply evaluate $\enc M\, \enc\istr$ with the Space KAM.
	
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\enc M\, \enc\istr\defeq\inits(\transs(\finals(\la \var\var)))\enc\istr 
		& 
		\stempty & \stempty & \too^*_{\bigo{\log(\size\istr)}}\text{ 
		(Lemma \ref{l:init})}\\
		\transs(\finals(\la \var\var)) & \stempty & 
		\initconfigs^{\kop} & \too^*_{\bigo{S_{\textrm{TM}}(\run) 
		+\log\size\istr}} \text{ 
		(Lemma \ref{l:trans})}\\
		\finals(\la\var\var) & \stempty & \configtwo^\kop & 
		\too^*_{\bigo{S_{\textrm{TM}}(\run) +\log\size\istr}} \text{ (Lemma 
		\ref{l:final})}\\
		\enc \bool & \stempty & \stempty
	\end{array}
	\]
\end{proof}

\paragraph{Init and Final.}


\begin{lemma}\label{l:init}
	$\spkamstate{\inits\,\cont\,\enc\inputstr}{ 
		\stempty}{\stempty}\tospkam^{\bigo{1}}\spkamstate\cont 
	\stempty{\initconfigs^{\kop}}$ and consumes space 
	$\Theta(\log(\size\inputstr))$.
\end{lemma}
\begin{proof}
	{\scriptsize\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\inits\,\cont\,\enc\inputstr & \stempty & \stempty \\
		\inits\,\cont & \stempty & (\enc\inputstr,\stempty)\\
		\inits\defeq(\la {d} \la {e} \la {f} \la{\cont'} \la{\inputstr'} 
		\cont'
		\tuple{\inputstr', d \csep e ,
			\cods{\elemblank}, f \csep 
			\cods{\statein}})\enc{\ntostr 
			0}\enc{\varepsilon} \enc{\varepsilon} & \stempty 
		& 
		\overbrace{(\cont,\stempty)}^{\cont^{\kop}}\cons 
		\overbrace{(\enc\inputstr,\stempty)}^{\enc\inputstr{^{\kop}}}&\too^3\\
		\la {d} \la {e} \la {f} \la{\cont'} \la{\inputstr'} 
		\cont' \tuple{\inputstr', d \csep e ,\cods{\elemblank}, f \csep 
			\cods{\statein}} & \stempty & 
		\overbrace{(\enc{\ntostr 0},\stempty)}
		^{\enc{\ntostr 0}^{\kop}}\cons 
		\overbrace{(\enc\ems,\stempty)}^{\enc{\ems}^{\kop}}
		\cons(\enc\ems,\stempty)\cons\cont^{\kop}\cons
		\enc\inputstr^{\kop} & \too^5\\
		\cont' \tuple{\inputstr', d \csep e ,\cods{\elemblank}, f \csep 
			\cods{\statein}} & \esub{\cont'} 
		{\cont^{\kop}}\cons\overbrace{\esub {\inputstr'} 
			{{\enc\inputstr}^{\kop}}\cons\esub d {\enc{\ntostr 0}^{\kop}} 
			\cons \esub e {\enc{\ems}^{\kop}}\cons \esub f 
			{\enc{\ems}^{\kop}}}^{\initconfigs^\env}  & 
		\stempty\\
		\cont' & \esub{\cont'} {\cont^{\kop}} & 
		(\tuple{\inputstr', d \csep e ,\cods{\elemblank}, f \csep 
			\cods{\statein}},\initconfigs^\env)\\
		\cont & \stempty & \underbrace{(\tuple{\inputstr', d \csep e 
				,\cods{\elemblank}, f \csep 
				\cods{\statein}},\initconfigs^\env)}_{\initconfigs^{\kop}}
	\end{array}
	\]}
	The space bound is immediate by inspecting the execution.
\end{proof}

\begin{lemma}\label{l:final} Let $\config$ be a final configuration, \ie 
	$\config\defeq(\inputstr,\counter,\str,\elem,\strtwo,\statefin)$ where 
	$\statefin\in\Statesfin$. Then
	\[\spkamstate{\finals(\la \var 
	\var)}\stempty{\config^\kop}\tospkam^{\bigo{1}}
	\begin{cases}
		\spkamstate{\la \var\la\vartwo\var}\stempty\stempty & \text{ if } 
		\statefin=\statefint\\
		\spkamstate{\la \var\la\vartwo\vartwo}\stempty\stempty & \text{ if } 
		\statefin=\statefinf
	\end{cases}\]
Moreover, the space consumption is $\Theta(\size{\config^\kop})$.
\end{lemma}
\begin{proof}
	We execute the Space KAM. Let us define $\tm\defeq\lambda 
	\inputstr'.\lambda n'.\lambda 
	\wstrl'.\lambda \elem'.\lambda 
	\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont'$.
	{\scriptsize\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\finals(\la \var \var) & \stempty & \config^\kop\\
		\finals\defeq\la {\cont'} \la {\config'}\config'\tm & \stempty & 
		(\la\var 
		\var,\stempty)\cons\config^\kop & \to^2\\
		\config'\tm & \esub{\config'}{\config^\kop}\cons\esub{\cont'}{(\la\var 
			\var,\stempty)} 
		& \stempty\\
		\config' & \esub{\config'}{\config^\kop} & (\tm,\esub{\cont'}{(\la\var 
			\var,\stempty)})\\
		\config^\kop\defeq\la\var\var fcm\cods\elem d\cods\statefin & \esub 
		f{(\enc\inputstr,\stempty)},\esub c {n^\kop}, \esub m {\str{^\kop}}, 
		\esub 
		d 
		{\strtwo^\kop} & (\tm,\esub{\cont'}{(\la\var 
			\var,\stempty)})\\
		\var fcm\cods\elem d\cods\statefin & \esub\var 
		{(\tm,\esub{\cont'}{(I,\stempty)})} \cons \esub 
		f{(\enc\inputstr,\stempty)},\esub c {n^\kop}, \esub m {\str{^\kop}}, 
		\esub 
		d 
		{\strtwo^\kop} & \stempty & \to^6\\
		\var & \esub\var {(\tm,\esub{\cont'}{(\la\var \var,\stempty)})} & 
		(\enc\inputstr,\stempty)\cons\counter^\kop\cons\str^\kop\cons 
		(\cods\elem,\stempty)\cons\strtwo^\kop\cons(\cods\statefin,\stempty)\\
		\tm\defeq\lambda 
		\inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont' & 
		\esub{\cont'}{(\la\var 
			\var,\stempty)} & 
		(\enc\inputstr,\stempty)\cons\counter^\kop\cons\str^\kop\cons 
		(\cods\elem,\stempty)\cons\strtwo^\kop\cons(\cods\statefin,\stempty)&\to^6\\
		q'N_1\ldots N_{\size{Q}}k' & \esub{\state'}{(\cods\statefin,\stempty)} 
		\cons 
		\esub{\cont'}{(\la\var \var,\stempty)} & \stempty&\to^{1+\size\States}\\
		\state' & \esub{\state'}{(\cods\statefin,\stempty)} & 
		(N_i,\stempty)_{1\leq 
			i\leq\size\States}\cons(\la\var \var,\stempty)\\
		\cods\statefin\defeq\lambda x_1\ldots\lambda x_{\size\States}.x_i & 
		\stempty & (N_i,\stempty)_{1\leq i\leq\size\States}\cons(\la\var 
		\var,\stempty)
	\end{array}
	\]}
	Two cases. If $\statefin=\statefint$, then:
	\[\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\cods\statefint\defeq\lambda x_1\ldots\lambda x_{\size\States}.x_i & 
		\stempty & (N_i,\stempty)_{1\leq i\leq\size\States}\cons(\la\var 
		\var,\stempty)&\to^{\size{\States}}\\
		\var_i & \esub{\var_i}{(N_i,\stempty)} & (\la\var \var,\stempty)\\
		N_i\defeq\la{\cont'}{\cont'(\la\var{\la\vartwo\var)}} & \stempty & 
		(\la\var \var,\stempty)\\
		{\cont'(\la\var{\la\vartwo\var})} & \esub{\cont'}{(\la\var 
			\var,\stempty)} & \stempty\\
		\cont' & \esub{\cont'}{(\la\var \var,\stempty)} & 
		(\la\var\la\vartwo\var,\stempty)\\
		\la\var \var & \stempty & (\la\var\la\vartwo\var,\stempty)\\
		\var & \esub{\var}{(\la\var\la\vartwo\var,\stempty)} & \stempty\\
		\la\var\la\vartwo\var & \stempty & \stempty
	\end{array}\]
	
	If $\statefin=\statefinf$, then:
	\[\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\cods\statefinf\defeq\lambda x_1\ldots\lambda x_{\size\States}.x_i & 
		\stempty & (N_i,\stempty)_{1\leq i\leq\size\States}\cons(\la\var 
		\var,\stempty)&\to^{\size{\States}}\\
		\var_i & \esub{\var_i}{(N_i,\stempty)} & (\la\var \var,\stempty)\\
		N_i\defeq\la{\cont'}{\cont'(\la\var{\la\vartwo\vartwo})} & \stempty & 
		(\la\var \var,\stempty)\\
		{\cont'(\la\var{\la\vartwo\vartwo})} & \esub{\cont'}{(\la\var 
			\var,\stempty)} & \stempty\\
		\cont' & \esub{\cont'}{(\la\var \var,\stempty)} & 
		(\la\var\la\vartwo\vartwo,\stempty)\\
		\la\var \var & \stempty & (\la\var\la\vartwo\vartwo,\stempty)\\
		\var & \esub{\var}{(\la\var\la\vartwo\vartwo,\stempty)} & \stempty\\
		\la\var\la\vartwo\vartwo & \stempty & \stempty
	\end{array}\]
	The space bound is immediate by inspecting the execution.
\end{proof}

\paragraph{Transition Function.}

\begin{lemma}
	$\spkamstate{\transs\,\cont}\stempty{\initconfigs^{\kop}}\tospkam^{\bigo{1}}\spkamstate{\theta}\stempty{(\theta,\stempty)\cons(\transaux,\stempty)\cons\cont^{\kop}
		\cons\initconfigs^{\kop}}$ in space $\bigo{\log(\size\istr)}$.
\end{lemma}

\input{./proofs/TM-to-SKAM/SKAM-transition}




\begin{proposition}[\SpKAM natural time overhead explosion]
	There is a family $\{\tm_{n}\}_{n\in\nat}$ of closed $\l$-terms such that its complete evaluation $\run_{n}:\tm_{n} \towh^{n} \tmtwo_{n}$ is simulated by \SpKAM runs $\runtwo_{n}$ taking both space and time exponential in $n$, that is, $\sizespace{\runtwo_{n}}=\sizetime{\runtwo_{n}}=\Omega(2^{n})$.
\end{proposition}

Before the main proof we need some preliminaries.

We define the following data structures:
\[
\begin{array}{rcl@{\hspace{2cm}}rcl}
	\lenv_0 & \defeq & \esub{\var_0}{(\Id,\stempty)} & \lenv_{n+1} & \defeq & 
	\esub{\var_{n+1}}{\stack_n}\cons\lenv_n
	\\[4pt]
	\stack_0 & \defeq & (\var_0\var_0,\lenv_0) & \stack_{n+1} & \defeq & 
	(\var_0..\var_{n+1},\lenv_{n+1})
\end{array}
\]
We observe that the size of $\lenv_{n}$ is exponential in $n$, since 
$\lenv_{n+1} \defeq \esub{\var_{n+1}}{\stack_n}\cons\lenv_n= 
\esub{\var_{n+1}}{(\var_0..\var_{n},\lenv_{n})}\cons\lenv_n$ \ie 
$\size{\lenv_{n+1}}\geq 2\size{\lenv_{n}}$ and thus $\size{\lenv_{n}}\geq2^n$.

We define $\ctx_n$ as follows:
\[
\begin{array}{rcl}
	\ctx_0 &\defeq& \lambda \var_0.\ctxhole(\var_0\var_0)
	\\
	\ctx_{n+1} &\defeq& 
	\lambda\var_{n+1}.\ctxhole(\var_0\ldots\var_{n+1})
\end{array}
\]
\begin{lemma}\label{l:counter-tr}
	If $\tm$ contains $\var_0,..,\var_n$ free, then 
	$\spkamstate{\ctx_0\ctxholep{\ctx_1\ctxholep{\cdots\ctx_{n} 
				\ctxholep{\tm}\cdots}}\Id} \stempty\stempty\tospkam^{\Theta(n)} 
	\spkamstate{\tm}{\lenv_n}{\stack_n}$.
\end{lemma}
\begin{proof}
	Case 0.
	\[\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\ctx_0\ctxholep\tm\Id & \stempty & 
		\stempty\\
		\ctx_0\ctxholep\tm\defeq\lambda \var_0.\tm(\var_0\var_0) & \stempty & 
		(\Id,\stempty)\\
		\tm(\var_0\var_0) & \esub{\var_0}{(\Id,\stempty)} & \stempty\\
		\tm & \esub{\var_0}{(\Id,\stempty)} & 
		(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})\\
	\end{array}\]
	
	Case $n+1$.
	
	We observe that $\ctx_0\ctxholep{\ctx_1\ctxholep{..\ctx_{n} 
			\ctxholep{\ctx_{n+1}\ctxholep\tm}..}}\Id$ can be rewritten to 
	$\ctx_0\ctxholep{\ctx_1\ctxholep{..\ctx_{n} 
			\ctxholep{\tmtwo}..}}\Id$ when 
			$\tmtwo\defeq\ctx_{n+1}\ctxholep\tm$. Of 
	course $\tmtwo$ contains $\var_0,..,\var_n$ free. We can thus apply the \ih.
	\[\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\ctx_0\ctxholep{\ctx_1\ctxholep{..\ctx_{n} 
				\ctxholep{\ctx_{n+1}\ctxholep\tm}..}}\Id & \stempty & 
		\stempty & \ih\\
		\ctx_{n+1}\ctxholep\tm\defeq\lambda \var_{n+1}.\tm(\var_0..\var_{n+1}) 
		& \lenv_n & \stack_n\\
		\tm(\var_0..\var_{n+1}) & \esub{\var_{n+1}}{\stack_n} \cons 
		\lenv_n=:\lenv_{n+1} & 
		\stempty\\
		\tm & \lenv_{n+1} & (\var_0..\var_{n+1},\lenv_{n+1})=:\stack_{n+1} \\
	\end{array}\]
	
	%	Case 1.
	%	\[\begin{array}{l|l|ll}
	%		\mathsf{Term}   & 
	%		\mathsf{Env} & \mathsf{Stack}\\
	%		\hhline{---}
	%		\ctx_0\ctxholep{\ctx_1\ctxholep\tm}\Id & \stempty & 
	%		\stempty\\
	%		\ctx_0\ctxholep{\ctx_1\ctxholep\tm}\defeq\lambda 
	%		\var_0.{\ctx_1\ctxholep\tm}(\var_0\var_0) & \stempty & 
	%		(\Id,\stempty)\\
	%		{\ctx_1\ctxholep\tm}(\var_0\var_0) & \esub{\var_0}{(\Id,\stempty)} 
	%& 
	%		\stempty\\
	%		{\ctx_1\ctxholep\tm}\defeq\la{\var_1}\tm(\var_0\var_1) & 
	%		\esub{\var_0}{(\Id,\stempty)} & 
	%		(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})\\
	%		\tm(\var_0\var_1) & 
	%		\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & \stempty\\
	%		\tm &  
	%\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & 
	%		
	%(\var_0\var_1,\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons
	%		 \esub{\var_0}{(\Id,\stempty)})
	%	\end{array}\]
	%
	%	Case 2.
	%	\[\begin{array}{l|l|ll}
	%		\mathsf{Term}   & 
	%		\mathsf{Env} & \mathsf{Stack}\\
	%		\hhline{---}
	%		(\lambda \var_0.\ctx_1\ctxholep{\ctx_2\ctxholep\tm}\var_0)\Id & 
	%		\stempty & 
	%		\stempty\\
	%		\lambda \var_0.\ctx_1\ctxholep{\ctx_2\ctxholep\tm}\var_0 & \stempty 
	%& 
	%		(\Id,\stempty)\\
	%		\ctx_1\ctxholep{\ctx_2\ctxholep\tm}\var_0 & 
	%		\esub{\var_0}{(\Id,\stempty)} & \stempty\\
	%		
	%\ctx_1\ctxholep{\ctx_2\ctxholep\tm}\defeq\la{\var_1}\ctx_2\ctxholep\tm(\var_0\var_1)
	%		 & 
	%		\esub{\var_0}{(\Id,\stempty)} & (\Id,\stempty)\\
	%		\ctx_2\ctxholep\tm(\var_0\var_1) & 
	%		\esub{\var_1}{(\Id,\stempty)}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & \stempty\\
	%		\ctx_2\ctxholep\tm\defeq\la{\var_2}\tm(\var_0\var_1\var_2) &  
	%		\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & 
	%		
	%(\var_0\var_1,\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons
	%		\esub{\var_0}{(\Id,\stempty)})\\
	%		\tm(\var_0\var_1\var_2) & 
	%		
	%\esub{\var_2}{(\var_0\var_1,\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons
	%			\esub{\var_0}{(\Id,\stempty)})} \cons 
	%		\esub{\var_1}{(\var_0\var_0,\esub{\var_0}{(\Id,\stempty)})}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & \stempty\\
	%		\tm & 
	%\esub{\var_2}{(\var_0\var_1,\esub{\var_1}{(\Id,\stempty)}\cons 
	%			\esub{\var_0}{(\Id,\stempty)})} \cons 
	%		\esub{\var_1}{(\Id,\stempty)}\cons 
	%		\esub{\var_0}{(\Id,\stempty)} & 
	%		
	%(\var_0\var_1\var_2,\esub{\var_2}{(\var_0\var_1,\esub{\var_1}{(\Id,\stempty)}\cons
	%			\esub{\var_0}{(\Id,\stempty)})} \cons 
	%		\esub{\var_1}{(\Id,\stempty)}\cons 
	%		\esub{\var_0}{(\Id,\stempty)})
	%	\end{array}\]
	
	
\end{proof}

Now we are able to prove the main Proposition.
\begin{proposition}[\SpKAM natural time overhead explosion]
	There is a family $\{\tm_{n}\}_{n\in\nat}$ of closed $\l$-terms such that there is a complete evaluation $\run_{n}:\tm_{n} \towh^{n} \tmtwo_{n}$ is simulated by \SpKAM runs $\runtwo_{n}$ taking both space and time exponential in $n$, that is, $\sizespace{\runtwo_{n}}=\sizetime{\runtwo_{n}}=\Omega(2^{n})$.
\end{proposition}
\begin{proof}
	We define $\tm_n$ as follows:
	\[
	\begin{array}{rcl}
		\tm_{n} &\defeq& \ctx_0\ctxholep{\ctx_1\ctxholep{\cdots\ctx_{n} 
				\ctxholep{\la{\vartwo} \Id}\cdots}}\Id
	\end{array}
	\]
	Now, we execute it.

	\[\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hhline{---}
		\tm_{n} \defeq 
		\ctx_0\ctxholep{\ctx_1\ctxholep{\cdots\ctx_{n-1}\ctxholep{\ctx_{n} 
		\ctxholep{\la{\vartwo} \Id}}\cdots}}\Id & \stempty & 
		\stempty & \text{Lemma~\ref{l:counter-tr}}\\
		\ctx_n\ctxholep{\la{\vartwo} \Id} \defeq 
		\lambda\var_{n}.(\la{\vartwo} \Id)(\var_0\ldots\var_{n}) & \lenv_{n-1} 
		& \stack_{n-1}\\
		(\la{\vartwo} \Id)(\var_0\ldots\var_{n}) & \lenv_n & \stempty\\
		\la{\vartwo} \Id& \stempty & \stack_n\\
		\Id & \stempty & \stempty
	\end{array}
	\]
	The space consumed (and thus also the low-level time) is exponential in $n$ 
	because the size of $\lenv_n$ is exponential in $n$.
\end{proof}


==> 99-scrolling.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Proofs of Section~\ref{sect:moving}}
\label{app:scrolling-tapes}

In the following we will often use the execution of the fix-point combinator. 
For this reason, we encapsulate its execution by the \SpKAM in a lemma. 
\begin{lemma}\label{l:fix}
	For each term $\tmtwo$,  
	$\spkamstate{\theta}\stempty{(\theta,\stempty)\cons(\tmtwo,\stempty)\cons\stack}
	 \tospkam^{\bigo{1}} 
	\spkamstate\tmtwo\stempty{\fix^{\kop}\cons\stack}$
	where $\fix^{\kop}\defeq(\var \var 
	\vartwo,\esub\vartwo{(\tmtwo,\lenv)}\cons\esub\var{(\theta,\stempty)})$ 
	consuming space $\bigo{\size\lenv+\size\stack+\log(\size\tmtwo)}$.
\end{lemma}
\begin{proof}
\[
\begin{array}{l|l|l}
	\mathsf{Term}   & 
	\mathsf{Env} & \mathsf{Stack}\\
	\hline
	\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo ) & \stempty & 
	(\theta,\stempty)\cons(\tmtwo,\stempty)\cons\stack\\
	\la\vartwo \vartwo(\var \var \vartwo ) & \esub\var{(\theta,\stempty)} & 
	(\tmtwo,\lenv)\cons\stack\\
	\vartwo(\var \var \vartwo ) & 
	\esub\vartwo{(\tmtwo,\lenv)}\cons\esub\var{(\theta,\stempty)} & 
	\stack\\
	\vartwo & \esub\vartwo{(\tmtwo,\lenv)} & \overbrace{(\var \var 
		\vartwo,\esub\vartwo{(\tmtwo,\lenv)}\cons\esub\var{(\theta,\stempty)})}^{\fix^{\kop}}\cons\stack\\
	\tmtwo & \lenv & \fix^{\kop}\cons\stack
\end{array}
\]
\end{proof}

We prove the following propositions in a top-down style, \ie required lemmata 
are below. This is done because otherwise lemmata statements would seem quite 
arbitrary.

\begin{proposition}
	Let $\strone\in\Bool^*$ and $\toy \defeq \fix (\la\varf\la 
	{\varthree}\varthree 
	\varf\varf \Id )$.
	\begin{enumerate}
		\item $\toy\, \encp\strone\Bool \towh^{\Theta(\size\strone)} \Id$.
		\item The \NaKAM evaluates $\toy\, 
		\encp\strone\Bool$ in 
		space 
		$\Omega(2^{\size\strone})$.
		\item The \SpKAM evaluates $\toy\, \encp\strone\Bool$ in space 
		$\Theta(\log\size\strone)$.
	\end{enumerate}
\end{proposition}
\begin{proof}\mbox{}
	\begin{enumerate}
		\item This point follows from the implementation theorem, applied to 
		the sequence of point 3.
		\item We prove the statement executing 
		$\toy\, \enc\strone$ with the \NaKAM. We set $\toyaux\defeq\la\varf\la 
		{\varthree}\varthree 
		\varf\varf \Id$.
		\[
		\begin{array}{l|l|ll}
			\mathsf{Term}   & 
			\mathsf{Env} & \mathsf{Stack}\\
			\hline
			\toy\, \enc\strone & \stempty & \stempty\\
			\toy\defeq\fix\toyaux  & \stempty & (\enc\strone,\stempty)\\
			\fix\defeq\theta\theta & \stempty & 
			(\toyaux,\stempty)\cons(\enc\strone,\stempty)\\
			\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo ) & 
			\stempty & (\theta,\stempty) \cons (\toyaux,\stempty) 
			\cons (\enc\strone,\stempty)\\
			\vartwo(\var \var \vartwo ) & \esub\var{(\theta,\stempty)}\cons 
			\esub \vartwo{(\toyaux,\stempty)}=:\lenv_0 & (\enc\strone,\stempty) 
			& 
			\text{Lemma~\ref{l:inv-kam-scrolling}}\\
			\Id & \lenvtwo_{\size\str} & \stempty
		\end{array}
		\]
		The space bound is proved since $\lenvtwo_{\size\str}$ is exponential 
		in $\size\str$.
		\item We prove the statement executing 
		$\toy\, \enc\strone$ with the \SpKAM. We set $\toyaux\defeq\la\varf\la 
		{\varthree}\varthree 
		\varf\varf \Id$.
		\[
		\begin{array}{l|l|ll}
			\mathsf{Term}   & 
			\mathsf{Env} & \mathsf{Stack}\\
			\hline
			\toy\, \enc\strone & \stempty & \stempty\\
			\toy\defeq\fix\toyaux  & \stempty & (\enc\strone,\stempty)\\
			\fix\defeq\theta\theta & \stempty & 
			(\toyaux,\stempty)\cons(\enc\strone,\stempty)\\
			\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo ) & 
			\stempty & (\theta,\stempty) \cons (\toyaux,\stempty) 
			\cons (\enc\strone,\stempty)\\
			\vartwo(\var \var \vartwo ) & \esub\var{(\theta,\stempty)}\cons 
			\esub \vartwo{(\toyaux,\stempty)}=:\lenv_0 & (\enc\strone,\stempty) 
			& 
			\text{Lemma~\ref{l:inv-spkam-scrolling}}\\
			\Id & \stempty & \stempty
		\end{array}
		\]
		The space bound is proved considering the bound in 
		Lemma~~\ref{l:inv-spkam-scrolling}.
	\end{enumerate}
\end{proof}
Let $\str\defeq\bool_1\ldots\bool_n\cons\ems$ be a string of length $n\geq 0$. 
Then, we can define 
$\lenv_i,\lenvtwo_i,\lenvthree_i$ for $0\leq i\leq n$ as follows:
\[
\begin{array}{rcl@{\hspace{2cm}}rcl}
	\lenv_0 &\defeq& \esub\var{(\theta,\stempty)}\cons 
	\esub \vartwo{(\toyaux,\stempty)} & \lenv_{i+1}&\defeq& 
	\esub\var{(\var,\lenv_i)}\cons 
	\esub \vartwo{(\vartwo,\lenv_i)}\\[4pt]
	\lenvtwo_{i}&\defeq& 
	\esub\varthree{(\enc{\bool_{i+1}..\bool_n\cons\ems},\lenvthree_{i})} 
	\cons\esub\varf{(\var \var \vartwo,\lenv_{i})}\\[4pt]
	\lenvthree_0&\defeq& \stempty& 
	\lenvthree_{i+1}&\defeq&\esub{\var_\ems}{(\Id,\lenvtwo_{i})} \cons 
	\esub{\var_1}{(\varf,\lenvtwo_{i})} \cons 
	\esub{\var_0}{(\varf,\lenvtwo_{i})}\cons\lenvthree_i
\end{array}\]

One can easy notice that the sizes of $\lenv_i,\lenvtwo_i,\lenvthree_i$ are 
exponential in $i$.

\begin{lemma}\label{l:inv-kam-scrolling}
	$\spkamstate{\vartwo(\var \var \vartwo 
	)}{\lenv_i}{(\enc\str,\lenvthree_i)}\tonakam^{\Omega(\size\str)} 
	\spkamstate{\Id}{\lenvtwo_{i+\size\str}}{\stempty}$
\end{lemma}
\begin{proof}
	By induction on the structure of $\str$.
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\vartwo(\var \var \vartwo ) & \lenv_i & (\enc\strone,\lenvthree_i)\\
		\vartwo & \lenv_i & (\var \var \vartwo,\lenv_i)\cons 
		(\enc\strone,\lenvthree_i)&\text{unfolding }\lenv_i\\
		\toyaux\defeq\la\varf\la 
		{\varthree}\varthree 
		\varf\varf \Id & \stempty & (\var \var \vartwo,\lenv_i)\cons 
		(\enc\strone,\lenvthree_i)\\
		\varthree \varf\varf \Id & 
		\esub\varthree{(\enc\strone,\lenvthree_i)}\cons\esub\varf{(\var \var 
			\vartwo,\lenv_i)}=:\lenvtwo_i & \stempty\\
		\varthree & 
		\esub\varthree{(\enc\strone,\lenvthree_i)}\cons\esub\varf{(\var \var 
			\vartwo,\lenv_i)} & (\varf,\lenvtwo_i) \cons (\varf,\lenvtwo_i) 
			\cons (\Id,\lenvtwo_i)\\
		\enc\strone & \lenvthree_i & (\varf,\lenvtwo_i) \cons 
		(\varf,\lenvtwo_i) 
		\cons (\Id,\lenvtwo_i)
	\end{array}
	\]
	Case $\str=\ems$.
	\[
	\begin{array}{l|l|l}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\enc\strone\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_\ems & 
		\lenvthree_i & (\varf,\lenvtwo_i) \cons (\varf,\lenvtwo_i) 
		\cons (\Id,\lenvtwo_i)\\
		\var_\ems & \esub{\var_\ems}{(\Id,\lenvtwo_i)} \cons 
		\esub{\var_1}{(\varf,\lenvtwo_i)} \cons 
		\esub{\var_0}{(\varf,\lenvtwo_i)}\cons \lenvthree_i & \stempty\\
		\Id & \lenvtwo_i & \stempty
	\end{array}
	\]
	Case $\str=\bool\cons\strtwo$.
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\enc\strone\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_b\enc\strtwo
		& \lenvthree_i & (\varf,\lenvtwo_i) \cons (\varf,\lenvtwo_i) 
		\cons (\Id,\lenvtwo_i)\\
		\var_\bool\enc\strtwo & \esub{\var_\ems}{(\Id,\lenvtwo_i)} \cons 
		\esub{\var_1}{(\varf,\lenvtwo_i)} \cons 
		\esub{\var_0}{(\varf,\lenvtwo_i)}\cons\lenvthree_i=:\lenvthree_{i+1} & 
		\stempty\\
		\var_\bool & \esub{\var_\ems}{(\Id,\lenvtwo_i)} \cons 
		\esub{\var_1}{(\varf,\lenvtwo_i)} \cons 
		\esub{\var_0}{(\varf,\lenvtwo_i)}\cons \lenvthree_i & 
		(\enc\strtwo,\lenvthree_{i+1})\\
		\varf & \esub\varthree{(\enc\strone,\lenvthree_i)}\cons\esub\varf{(\var 
			\var \vartwo,\lenv_i)} & (\enc\strtwo,\lenvthree_{i+1})\\
		\var \var \vartwo & \esub{\var}{(\var,\lenv_{i-1})} \cons 
		\esub{\vartwo}{(\vartwo,\lenv_{i-1})} & (\enc\strtwo,\lenvthree_{i+1})\\
		\var &  \esub{\var}{(\var,\lenv_{i-1})} \cons 
		\esub{\vartwo}{(\vartwo,\lenv_{i-1})} & (\var,\lenv_i) 
		\cons(\vartwo,\lenv_i) \cons (\enc\strtwo,\lenvthree_{i+1}) & 
		\text{unfolding }\lenv_{i-1}\\
		\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo ) & 
		\stempty & (\var,\lenv_i) 
		\cons(\vartwo,\lenv_i) \cons (\enc\strtwo,\lenvthree_{i+1})\\
		\vartwo(\var \var \vartwo ) & \esub{\var}{(\var,\lenv_i)} \cons 
		\esub{\vartwo}{(\vartwo,\lenv_i)}=:\lenv_{i+1} & 
		(\enc\strtwo,\lenvthree_{i+1}) & \ih\\
		\Id & \lenvtwo_{i+\size\str} & \stempty
	\end{array}
	\]
\end{proof}

\begin{lemma}\label{l:inv-spkam-scrolling}
	The \SpKAM executes the reduction $\spkamstate{\vartwo(\var \var \vartwo 
		)}{\lenv_0}{(\enc\str,\stempty)}\tospkam^{\Theta(\size\str)} 
	\spkamstate{\Id}{\stempty}{\stempty}$ consuming $\bigo{\log(\size\str)}$ 
	space.
\end{lemma}
\begin{proof}
	By induction on the structure of $\str$.
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\vartwo(\var \var \vartwo ) & \lenv_0 & (\enc\strone,\stempty)\\
		\vartwo & \esub \vartwo{(\toyaux,\stempty)} & (\var \var 
		\vartwo,\lenv_0)\cons 
		(\enc\strone,\stempty)\\
		\toyaux\defeq\la\varf\la {\varthree}\varthree 
		\varf\varf \Id & \stempty & (\var \var \vartwo,\lenv_0)\cons 
		(\enc\strone,\stempty)\\
		\varthree \varf\varf \Id & 
		\esub\varthree{(\enc\strone,\stempty)}\cons\esub\varf{(\var \var 
			\vartwo,\lenv_0)} & \stempty\\
		\varthree & 
		\esub\varthree{(\enc\strone,\stempty)} & (\var \var \vartwo,\lenv_0) 
		\cons (\var \var 
			\vartwo,\lenv_0) 
		\cons (\Id,\stempty)\\
		\enc\strone & \stempty & (\var \var \vartwo,\lenv_0) 
		\cons (\var \var 
		\vartwo,\lenv_0) 
		\cons (\Id,\stempty)
	\end{array}
	\]
	Case $\str=\ems$.
	\[
	\begin{array}{l|l|l}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\enc\strone\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_\ems & 
		\stempty & (\var \var \vartwo,\lenv_0) 
		\cons (\var \var 
		\vartwo,\lenv_0) 
		\cons (\Id,\stempty)\\
		\var_\ems & \esub{\var_\ems}{(\Id,\stempty)}  & \stempty\\
		\Id & \stempty & \stempty
	\end{array}
	\]
	Case $\str=\bool\cons\strtwo$.
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term}   & 
		\mathsf{Env} & \mathsf{Stack}\\
		\hline
		\enc\strone\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_b\enc\strtwo
		& \stempty & (\var \var \vartwo,\lenv_0) 
		\cons (\var \var \vartwo,\lenv_0) \cons (\Id,\stempty)\\
		\var_\bool\enc\strtwo & \esub{\var_b}{(\var \var \vartwo,\lenv_0)}  & 
		\stempty\\
		\var_\bool & \esub{\var_b}{(\var \var \vartwo,\lenv_0)} & 
		(\enc\strtwo,\stempty)\\
		\var \var \vartwo & \lenv_0 & (\enc\strtwo,\stempty)\\
		\var &  \esub{\var}{(\theta,\stempty)} & (\theta,\stempty) 
		\cons(\toyaux,\stempty) \cons (\enc\strtwo,\stempty) \\
		\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo ) & 
		\stempty & (\theta,\stempty) 
		\cons(\toyaux,\stempty) \cons (\enc\strtwo,\stempty)\\
		\vartwo(\var \var \vartwo ) & \lenv_0 & 
		(\enc\strtwo,\stempty) & \ih\\
		\Id & \stempty & \stempty
	\end{array}
	\]
	The space bound is proved since there is a static bound (8) on the number 
	of closures during the execution.
\end{proof}

\begin{proposition}
	Let $\strone\in\Bool^*$ and $\globalcopy \defeq \la\varthree(\fix 
	(\la\varf\la 
	{\strone'}\strone' \varf\varf \varthree) \varthree)$.
	\begin{enumerate}
		\item $\globalcopy\, \encp\strone\Bool \towh^{\Theta(\size\strone)} 
		\encp\strone\Bool$.
		\item The space used by the \SpKAM to simulate the evaluation of the 
		previous point is $\Theta(\log\size\strone)$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	We prove the second point of the statement by directly executing the 
	\SpKAM. The first point is then obtained as a corollary using the complexity 
	and correctness properties of the \SpKAM. Since $\Bool$ is the only 
	alphabet that we are using, we remove all the superscripts. Let us define 
	$\tm\defeq\la\varf\la 
	{\strone'}\strone' \varf\varf \varthree$. 
	
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term} & \mathsf{Environment} & \mathsf{Stack}\\ 
		\cline{1-3}
		\globalcopy\, \enc\strone & \stempty & \stempty & \to\\
		\globalcopy\defeq\la\varthree(\fix \tm \varthree) & \stempty & 
		(\enc\strone,\stempty)=:\str^\kop & \to\\
		\fix \tm \varthree & \esub\varthree{\str^\kop} & 
		\stempty & \to\\
		\fix \tm & \esub\varthree{\str^\kop} & \str^\kop & \to\\
		\fix\defeq \theta \theta & 
		\stempty & (\tm,\esub\varthree{\str^\kop}) \cons \str^\kop & \to\\
		\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo) & \stempty & 
		(\theta,\stempty) \cons (\tm,\esub\varthree{\str^\kop}) \cons \str^\kop 
		& \to^{\Theta(\size{\str})}(\text{ Lemma~\ref{l:global}})\\
		\enc\str & \stempty & \stempty
	\end{array}
	\]
\end{proof}
\begin{lemma}\label{l:global}
	Let $\strone\in\Bool^*$ and $\tm\defeq\la\varf\la 
	{\strone'}\strone' \varf\varf \varthree$. Then 
	$\spkamstate{\theta}{\stempty}{(\theta,\stempty) \cons 
	(\tm,\esub\varthree{(\tmtwo,\lenv)}) \cons 
	\str^\kop}\tospkam^{\Theta(\size{\str})}\spkamstate{\tmtwo}{\lenv}{\stempty}$
	 and moreover the space used is 
	 $\bigo{\size\lenv+\log\size{\str}+\log\size{\tmtwo}}$.
\end{lemma}
\begin{proof}
	We proceed by induction on the 
	structure of $\str$. The first steps are common to both the base case and 
	the induction step. We define $\fix^\kop\defeq(\var\var\vartwo, 
	\esub\vartwo{(\tm,\esub\varthree{(\tmtwo,\lenv)})} \cons 
	\esub\var{(\theta,\stempty)})$.
	
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term} & \mathsf{Environment} & \mathsf{Stack}\\ 
		\cline{1-3}
		\theta\defeq\la\var \la\vartwo \vartwo(\var \var \vartwo) & \stempty & 
		(\theta,\stempty) \cons (\tm,\esub\varthree{(\tmtwo,\lenv)}) \cons 
		\str^\kop 
		& \to(\text{ Lemma~\ref{l:fix}})\\
		\tm\defeq\la\varf\la 
		{\strone'}\strone' \varf\varf \varthree & 
		\esub\varthree{(\tmtwo,\lenv)} & 
		\fix^\kop \cons \str^\kop & \to^2\\
		\strone' \varf\varf \varthree & \esub\varf{\fix^\kop} 
		\cons\esub{\strone'}{\str^\kop}\cons \esub\varthree{(\tmtwo,\lenv)} & 
		\stempty & \to^3\\
		\strone' & \esub{\strone'}{\str^\kop} & \fix^\kop \cons \fix^\kop \cons 
		(\tmtwo,\lenv) & \to\\
		\enc\str & \stempty & \fix^\kop \cons \fix^\kop \cons 
		(\tmtwo,\lenv)
	\end{array}
	\]
	
	Base case: $\str=\ems$.
	
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term} & \mathsf{Environment} & \mathsf{Stack}\\ 
		\cline{1-3}
		\enc\str\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_\ems & \stempty 
		& \fix^\kop \cons \fix^\kop \cons (\tmtwo,\lenv) & \to^4\\
		\tmtwo & \lenv & \stempty
	\end{array}
	\]
	
	Inductive case: $\str:b\cons\strtwo$ where $b\in\{0,1\}$.
	
	\[
	\begin{array}{l|l|ll}
		\mathsf{Term} & \mathsf{Environment} & \mathsf{Stack}\\ 
		\cline{1-3}
		\enc\str\defeq\la{\var_0}\la{\var_1}\la{\var_\ems}\var_b\enc\strtwo & 
		\stempty 
		& \fix^\kop \cons \fix^\kop \cons (\tmtwo,\lenv) & \to^3\\
		\var_b\enc\strtwo & \esub{\var_b}{\fix^\kop} & \stempty & \to\\
		\var_b & \esub{\var_b}{\fix^\kop} & (\enc\strtwo,\stempty)=: 
		\strtwo^\kop & \to\\
		\var \var \vartwo & \esub\vartwo{(\tm,\esub\varthree{(\tmtwo,\lenv)})} 
		\cons 
		\esub\var{(\theta,\stempty)} & \strtwo^\kop & \to^2\\
		\var & \esub\var{(\theta,\stempty)} & (\theta,\stempty) \cons 
		(\tm,\esub\varthree{(\tmtwo,\lenv)}) \cons \strtwo^\kop & \to\\
		\theta & \stempty & (\theta,\stempty) \cons 
		(\tm,\esub\varthree{(\tmtwo,\lenv)}) \cons \strtwo^\kop & 
		\to^{\Theta(\size\strtwo)} 
		\text{ \ih}\\
		\tmtwo & \lenv & \stempty
	\end{array}
	\]
	
	About space, it is immediate to see that all computations are constrained 
	in space $\bigo{\size\lenv+\log\size{\str}+\log\size{\tmtwo}}$, since at 
	any point 
	during the computation there is a \emph{bounded} number of closures, 
	independent from both $\str$ and $\tmtwo$.
\end{proof}

==> 99-time-spkam.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%
\section{Proofs of Section~\ref{sect:time-spkam}}\label{app:time}
\begin{theorem}[TMs are simulated by the \SpKAM in reasonable low-level time]
	\hfill
	\begin{enumerate}
		\item Every TM run $\run$ can be simulated by the \SpKAM in time 
		$\bigo{poly(\size\run)}$.
		\item Every \SpKAM run $\exec: \compil\tm \tospkam^{*} \state$  can be 
		implemented on RAM in time $\bigo{\sizetime{\run}}$.
		\item \ccbn evaluation $\towh$ and the time of the \SpKAM provide a 
		reasonable time cost model for the $\l$-calculus.
	\end{enumerate}
\end{theorem}
\begin{proof}
	The first point is the only one which is non-trivial. We have already 
	proved that the Space KAM can simulate TMs runs $\run$ in a number of 
	\emph{transitions} which is polynomial in $\size\run$. However, this does 
	not 
	necessarily means that the (low-level) time is also polynomial in $\run$, 
	see Proposition~\ref{prop:spkam-not-reas-for-nat-time}. About the execution 
	of terms which are the image of the encoding of TMs into the $\l$-calculus, 
	we can say however that the overhead stays polynomial. Indeed, the 
	exponential blowup comes from the fact that environments are duplicated in 
	an uncontrolled way. This does not happen in the execution of the encoding 
	of TMs, where duplication is restrained to the fix-point operator and to 
	the input components of the state. In other words, we duplicate only 
	objects of fixed size, thus confirming the polynomial bound.
	
	There is another, indirect, way of proving the same results. If the 
	(low-level) time were exponential in $\size\run$, then the space should be 
	at least linear in $\size\run$\footnote{This is because space cannot be 
	less than logarithmic in time.}. But we have proved that this is not the 
	case since space is linearly related with the \emph{space} consumption of 
	$\run$, and \emph{not} with its length.
\end{proof}

\subsection{\TiKAM}

\begin{theorem}
	Let $\run: \compil{\tm_{0}} \totikam^{*} \state$ be a complete \TiKAM run. 
	It can 
	be implemented on RAM in time and space
	$\bigo{\sizeb\run\cdot\log(\sizeb\run\cdot\size{\tm_0})}$.
\end{theorem}
\begin{proof}
	Since the \TiKAM is implemented \emph{with} unchaining, the number of 
	transitions of complete runs is $\bigo{\sizeb\run}$. The cost of each 
	transition can be bounded by $\log(\sizeb\run\cdot\size{\tm_0})$ since in 
	any transition a constant number of pointers to the code and pointers to 
	data structures are manipulated. About space, new closures/environments, 
	costing $\log(\sizeb\run\cdot\size{\tm_0})$, are created in any transition, 
	except for $\tokamsub$. Thus also space consumption is 
	$\bigo{\sizeb\run\cdot\log(\sizeb\run\cdot\size{\tm_0})}$.
\end{proof}

==> machines/NaiveKAM-cost.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../main.tex
%%%%%%%%%%%%%%

\begin{array}{cc}
		\begin{array}{ccccccccccc}
			\textsc{Terms}
			&
			\textsc{Closures}
			&
			\textsc{States}
			\\
			\size{\tmtwo}  \defeq \log{\size{\tm_{0}}}
			&
			\size{(\tmtwo,\lenv)}  \defeq  \size\tmtwo+\size\lenv
			&
			\size{(\tmtwo,\lenv,\stack)} \defeq  \size\tmtwo+\size\lenv+\size{\stack}

			\\[6pt]
			
			\textsc{Stacks}
			&
			\textsc{Environments}
			&
			\textsc{Transitions $\state \tomach \statetwo$}
			\\
			\begin{array}{r@{\hspace{.2cm}}c@{\hspace{.2cm}}l}
			\size{\stempty} & \defeq &0
			\\
			 \size{\clos\cdot\stack} & \defeq &	\size{\clos}+\size{\stack}
			\end{array}
			&
						\begin{array}{r@{\hspace{.2cm}}c@{\hspace{.2cm}}l}
			\size{\stempty} & \defeq & 0
			\\
			\size{\esub\var\clos\cdot\lenv} & \defeq & \size\var + \size{\clos}+\size\lenv
			\end{array}
		&
		\begin{array}{r@{\hspace{.2cm}}c@{\hspace{.2cm}}l@{\hspace{.5cm}}r@{\hspace{.2cm}}c@{\hspace{.2cm}}l}
		\sizetime{\tomach} & \defeq & poly(\size\state)
%		\sizetime{\tokamsea} & \defeq & \bigo{\size\state}
%		&\sizesp{\tokamsea} & \defeq & \bigo{\size\lenv}
		\\
%		\sizetime{\tokamb} & \defeq & \bigo{\size\state}
%		&\sizesp{\tokamb} & \defeq & \bigo{1}
%		\\
%		\sizetime{\tokamsub} & \defeq & \bigo{\size\lenv}
%		&\sizesp{\tokamsub} & \defeq & \bigo{1}
		\end{array}
		\end{array}
		\end{array}


==> machines/SharingKAM-cost.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
\begin{tabular}{cc}
		$
		\begin{array}{ccccccccccc}
			\textsc{Transitions} &\textsc{States}\\
			\sizetime{\tomach}  \defeq  \log(\sizeb\run)\cdot\log(\size{\tm_0}) & \size{(\tmtwo,\lenv,\stack, \heap)} \defeq  \size\tmtwo+\size\lenv+\size{\stack} + \size\heap\\[4pt]
			\textsc{Terms}
			&
			\textsc{Closures}
			\\
			\size{\tmtwo}  \defeq \log{\size{\tm_{0}}}
			&
			\size{(\tmtwo,\lenv)}  \defeq  \size\tmtwo+\size\lenv
			\\[6pt]
			
			\textsc{Stacks}
			&
			\textsc{Heaps}
			\\
			\begin{array}{c}
			\size{\stack}  \defeq \log{\sizeb\run}
			\\
			\textsc{Environments}
			\\
			\size{\lenv}  \defeq \log{\sizeb\run}
			\end{array}
			&
			\begin{array}{r@{\hspace{.2cm}}c@{\hspace{.2cm}}l}
			\size{\stempty}  &\defeq& 0
			\\
			\size{\{\stack{\defeq} \clos{\cons}\stacktwo\} \uplus \heap}  
			&\defeq& \size\clos + \size\stacktwo +\size\heap
			\\
			\size{\{\lenv{\defeq} \esub\var\clos{\cdot}\lenvtwo\} \uplus\heap} 
			&\defeq& \size{\var} + \size\clos + \size\lenvtwo + \size\heap
			\end{array}
		%\sizetime{\tokamsea} & \defeq & \bigo{\log{\sizeb\run}+\log{\size{\tm_0}}}
		%&\sizesp{\tokamsea} & \defeq & \bigo{\log{\sizeb\run}}
		\\[20pt]
		%\sizetime{\tokamb} & \defeq & \bigo{\log{\sizeb\run}+\log{\size{\tm_0}}}
		%&\sizesp{\tokamb} & \defeq & \bigo{\log{\sizeb\run}}
		%\\
		%\sizetime{\tokamsub} & \defeq & 
		%\bigo{\log{\sizeb\run}+\size{\tm_{0}}\cons\log{\size{\tm_0}}}
		%&\sizesp{\tokamsub} & \defeq & \bigo{1}
\end{array}$
		\end{tabular}

==> machines/SharingKAM.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../main.tex
%%%%%%%%%%%%%%

	
$\begin{array}{c}\begin{array}{c@{\hspace{.7cm}}c@{\hspace{.7cm}}c@{\hspace{.7cm}}c@{\hspace{.7cm}}c}
	\textsc{Closures} &
	\textsc{Environments}&
	\textsc{Stacks} & \textsc{States}\\
	\clos  \grameq  (\tm,\lenv) &  \lenv  &
	\stack  & \state\grameq(\tm,\lenv,\stack, \heap)
	\end{array}\\[4pt]
	\begin{array}{c}
	\textsc{Heaps}
	\\
	\heap \grameq \stempty \midd \{\stack^*\defeq \clos{\cons}\stacktwo\} \uplus 
	\heap \midd \{\lenv^*\defeq \esub\var\clos{\cdot}\lenvtwo\} \uplus\heap \qquad (\cdot)^* = \text{fresh}
	\end{array}\\[10pt]
	\hhline{=}\\[-8pt]
	\begin{array}{
			l@{\hspace{.2cm}}l@{\hspace{.2cm}}l@{\hspace{.4cm}}l | l |
			l@{\hspace{.4cm}}l@{\hspace{.4cm}}@{\hspace{.4cm}}llll}
		%	\newcommand{\kstatetab}[4]{&\red{#1} && #2 && #3 && #4 }
		\mathsf{Term} &  \mathsf{Env} & \mathsf{Stk} & \mathsf{Heap}
		&&	\mathsf{Term}  & \mathsf{Env} & \mathsf{Stack}& \mathsf{Heap}
		\\
		\cline{1-10}
					&&&&\\[-8pt]
		\shkstatetab{ \tm\var }{ \lenv }{ \stack }{ \heap } &
		\tokamseav &%\\[-2pt]
		\shkstatetab{ \tm }{ \lenv }{ \stacktwo }{ \{\stacktwo \defeq 
			\lenv(\var){\cons}\stack\} \uplus \heap }
		\\[3pt]	
		\shkstatetab{ \tm\tmtwo }{ \lenv }{ \stack }{ \heap } \qquad\quad \tmtwo\not\in\mathcal{V}&
		\tokamseanv &%\\[-2pt]
		\shkstatetab{ \tm }{ \lenv }{ \stacktwo }{ \{\stacktwo \defeq 
		(\tmtwo,\lenv){\cons}\stack\} \uplus \heap } 
		\\[3pt]				
		\shkstatetab{ \la\var\tm }{ \lenv }{ \stack }{ \{\stack \defeq 
		\clos{\cons}\stacktwo \}\uplus \heap } &
		\tokamb &%\\[-2pt]
		\shkstatetab{ \tm }{ \lenvtwo }{ \stacktwo }{ \{\lenvtwo \defeq \esub\var 
		\clos{\cons} \lenv\} \uplus \heap }
		\\[3pt]  
		\shkstatetab{ \var }{ \lenv }{ \stack }{ \heap } &
		\tokamsub &%\\[-2pt]
		\shkstatetab{ \tmtwo}{ \lenvtwo }{\stack }{ \heap } \quad \mbox{if 
		}\lenv(\var) = (\tmtwo,\lenvtwo)
%		\\[3pt]
%		\cline{1-9}
		\end{array}\\[3pt]
		\hhline{=}\\[-8pt]
		\input{machines/SharingKAM-cost}
\end{array}$


==> machines/outKAM.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
\begin{center}
	\fbox{
	$\begin{array}{c}
	\begin{array}{c@{\hspace{.5cm}}c@{\hspace{.5cm}}c@{\hspace{.5cm}}c}
	\textsc{Closures} &
	\textsc{Environments} &\textsc{Stacks}&
	\textsc{States}
	\\
	\clos  \grameq  (\tm,\lenv) &  \lenv  \grameq  \stempty \midd \esub\var \clos\cdot \lenv & \stack  
	\grameq  \stempty \midd \clos\cdot \stack&
	\state\grameq(\tm,\lenv,\stack)
	\\\\
	
	\end{array}
	\\
	\begin{array}{
			l@{\hspace{.4cm}}l@{\hspace{.4cm}}l | l |
			l@{\hspace{.4cm}}l@{\hspace{.4cm}}lll}
		%	\newcommand{\kstatetab}[4]{&\red{#1} && #2 && #3 && #4 }
		\mathsf{Term} &  \mathsf{Env} & 
		\mathsf{Stack}
		&&	\mathsf{Term}  & \mathsf{Env} 
		& 
		\mathsf{Stack}
		\\
		\cline{1-8}
		&&&&\\[-8pt]
		\kstatetab{ \tm\tmtwo }{ \lenv }{ \stack } &
		\tokamsea &%\\[-2pt]
		\kstatetab{ \tm }{ \lenv }{ (\tmtwo,\lenv)\cons \stack }
		\\[3pt]				
		\kstatetab{ \la\var\tm }{ \lenv }{ \clos\cons \stack } &
		\tokamb &%\\[-2pt]
		\kstatetab{ \tm }{ \esub\var \clos\cons \lenv }{ \stack }
		\\[3pt]  
		\kstatetab{ \var }{ \lenv }{ \stack } &
		\tokamsub &%\\[-2pt]
		\kstatetab{ \tmtwo}{ \lenvtwo }{\stack } & \mbox{if }\lenv(\var) = (\tmtwo,\lenvtwo)
		\\[3pt]
		%\cline{1-7}
		\end{array}\\[30pt]
	\hhline{=}\\[-3pt]
	\input{machines/NaiveKAM-cost}
	\end{array}$
	}
\end{center}


==> proofs/TM-to-lambda/final-proof.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	Define
	\begin{align*}
		\finals &\defeq \la {\cont'} \la {\config'}\config'(\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont')
	\end{align*}
	where:
	\[
	N_i\defeq\begin{cases}
	\la{\cont'}{\cont'(\la\var{\la\vartwo\var)}} &\text{ if }q_i= \statefint\\
	\la{\cont'}{\cont'(\la\var{\la\vartwo\vartwo)}} &\text{ if }q_i= \statefinf\\
	\mbox{whatever closed term (say, the identity)} &\text{ otherwise }
	\end{cases}
	\]
	Then:
	\[\begin{array}{rclcl}
	\finals\, \cont\, \enc\config
	& = &
	(\la {\cont'} \la {\config'}\config'(\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont')
) \cont \enc\config\\
	& \tobdet^2 &
	\enc\config(\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont)\\
	& = &
	\enc{ (\inputstr,\counter \csep \wstrl, \elem, \wstrr \csep \state) }(\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont)\\
	& = &
	(\lambda 
	x.x\encp{\inputstr}{\Bool^*}\enc{\ntostr\counter}\; 
	\encp{\wstrl^{\rop}}{\Boolb^*}\; 
	\cod{\elem}{\Boolb}\;\encp{\wstrr}{\Boolb^*}\;\cod{\state}{\States})
	 (\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont)\\
	& \tobdet &
	(\lambda \inputstr'.\lambda n'.\lambda 
		\wstrl'.\lambda \elem'.\lambda 
		\wstrr'.\lambda \state'. \state' N_1\ldots N_{\size{\States}}\cont) 
	\encp{\inputstr}{\Bool^*}\enc{\ntostr\counter}\;\encp{\wstrl^{\rop}}{\Boolb^*} 
	\; 
	\cod{\elem}{\Boolb}\;\encp{\wstrr}{\Boolb^*}\;\cod{\state}{\States}\\
	 
	&\tobdet^6 &
	\cod{\state}{\States} N_1\ldots N_{\size{\States}}\cont
	\\&=&
	(\la{\var_1\ldots\var_{\size\States}}{\var_j})N_1\ldots N_{\size{\States}}\cont\\ 
	&\tobdet^{\size\States}&N_j\cont
	\end{array}\]
	If $\state=\statefint$, then:
	\[\begin{array}{rclcl}
	N_j\cont & = & (\la{\cont'}{\cont'(\la\var{\la\vartwo\var})})\cont\\
	&\tobdet&\cont(\la\var{\la\vartwo\var})
	\end{array}\]
	If $\state=\statefinf$, then:
	\[\begin{array}{rclcl}
	N_j\cont & = & (\la{\cont'}{\cont'(\la\var{\la\vartwo\vartwo})})\cont\\
	&\tobdet&\cont(\la\var{\la\vartwo\vartwo})
	\end{array}\]
\end{proof}

==> proofs/TM-to-lambda/init-proof.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	Define
	\[
		\inits \defeq (\la {d} \la {e} \la {f} \la{\cont'} \la{\inputstr'} 
		\cont'
		\tuple{\inputstr', d \csep e ,
			\cod{\elemblank}{\Boolb}, f \csep 
			\cod{\statein}{\States}})\enc{\ntostr 
			0}\encp{\varepsilon}{\Boolb^*} \encp{\varepsilon}{\Boolb^*}
	\]
	Please note that the term is not in normal form. This is for technical 
	reasons that will be clear next.
	Then 
	\[\begin{array}{rclcl}
	\inits\, \cont\, \encp\inputstr{\Boolin^*}
	& = &
	(\la {d} \la {e} \la {f} \la{\cont'} \la{\inputstr'} 
	\cont'
	\tuple{\inputstr', d \csep e ,
		\cod{\elemblank}{\Boolb}, f \csep 
		\cod{\statein}{\States}})\enc{\ntostr 
		0}\encp{\varepsilon}{\Boolb^*} \encp{\varepsilon}{\Boolb^*} \cont 
		\encp\inputstr{\Boolin^*}\\
	& \tobdet^5 &
	\cont\, 
	\tuple{\encp{\inputstr}{\Boolin^*},\enc{\ntostr 0} \csep 
	\encp{\varepsilon}{\Boolb^*},
		\cod{\elemblank}{\Boolb}, \encp{\varepsilon}{\Boolb^*} \csep
		\cod{\statein}{\States}}\\
	& = &
	\cont\, \enc{(\inputstr,0 \csep \varepsilon, \elemblank, \ems \csep \statein)}\\
	& = &
	\cont\, \enc\initconfigs
	\end{array}\]
\end{proof}

==> proofs/TM-to-lambda/one-step-simulation-proof.tex <==
% !TeX spellcheck = en_US
% !TEX root = ../../main.tex
The transition function $\delta(\bool,\elem,\state)$ is a 3-dimensional table having for coordinates:
\begin{itemize}
\item the current bit $\bool$ on the input tape, which is actually retrieved 
from the input tape $i$ and the counter $n$ of the current input position,
\item the current character $\elem$ on the work tape, and 
\item the current state $\state$, 
\end{itemize}
The transition function is encoded as a recursive $\l$-term $\transs$ taking as argument the encodings of $\istr$, and $\counter$---to retrieve $\bool$---and $\elem$ and $\state$. It works as follows:
\begin{itemize}
\item It first retrieves $\bool$ from $\counter$ and $\istr$ by applying the $\lookupl$ function;
\item It has a subterm $A_{\bool}$ for the four values of $\bool$. The right 
sub-term is selected by applying the encoding $\cods\bool$ of $\bool$ to 
$A_{0},A_{1},A_\stsym$ and $A_\ensym$.

\item Each $A_{\bool}$ in turn has a sub-term $B_{\bool,\elem}$ for every character $\elem\in \Boolb$, corresponding to the working tape coordinates. The right sub-term is selected by applying the encoding $\cods\elem$ of  the current character $\elem$ on the work tape to $B_{\bool,0}, B_{\bool,1}, B_{\bool, \elemblank}$.

\item Each $B_{\bool,\elem}$ in turn has a subterm $C_{\bool,\elem,\state}$ for every character $\state$ in $\States$. The right sub-term is selected by applying the encoding $\cods\state$ of  the current state $\state$ to $C_{\bool,\elem,\state_{1}}, \ldots, B_{\bool, \elem,\state_{\size\States}}$.

\item The subterm $C_{\bool,\elem,\state}$ produces the (encoding of the) next configuration according to the transition function $\delta$. If $\delta$ decreases (resp. increases) the counter for the input tape then $C_{\bool,\elem,\state}$ applies $\predl$ (resp. $\succl$) to the input counter and then applies a term corresponding to the required action on the work tape, namely:
\begin{itemize}
	\item $S$ (for \emph{stay}) if the head does not move. This case is easy, $S$ simply produces the next configuration.
	\item $L$ if it moves left. Let $\wstrl = \wstr\elem''$, $\elem'$ the element that the transition has to write and $\state'$ the new state. Then $L$ has a subterm $L_{\elem''}^{\elem',\state'}$ for each $\elem''\in\Boolb$ the task of which is to add $\elem'$ to the right part of the work tape, remove $\elem''$ from the left part of the work tape (which becomes $\wstr$), and make $\elem''$ the character in the work head position.
	\item $R$ if it moves right. Its structure is similar to the one of $L$.
\end{itemize}
In order to be as modular as possible we use the definition of $S$, $L$, and $R$ for the cases when the input head moves also for the cases where it does not move, even if this requires a useless (but harmless) additional update of the counter $\counter$.
\end{itemize}

Define
\[\begin{array}{rclll}
\transaux 
& \defeq & 
\lambda \var.\la{\cont'}\lambda \config'.\config'(\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K \istr' \counter')
\\

%\transaux 
%& \defeq & 
%(\lambda x.\la{\cont'}\lambda \config'.\config'(\lambda i.\lambda n.\lambda u.\lambda a.\lambda 
%v.\lambda q.q M_1\ldots M_{\size\States} au\cont v)),
\\
\transs 
& \defeq &
\fix \transaux,
\end{array}\]
where:
\[\begin{array}{rcl}
K & \defeq & \la {\bool'} \bool'\, 
A_{0}A_{1}A_{\stsym}A_{\ensym}\elem'\state'\var \cont' \istr' \counter'\wstrl' 
\wstrr'
\\
A_{\bool} & \defeq & \la{\elem'} \elem' B_{\bool,0} B_{\bool,1} B_{\bool,\elemblank} 
\\\\
B_{\bool,\elem} & \defeq & \la{\state'}\state' C_{\bool,\elem,\state_{1}}\ldots C_{\bool,\elem,\state_{\size\States}}
\\
% \la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 

C_{\bool,\elem,\state}&\defeq&
\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'}
    \left\{
   \begin{array}{ll}
	\cont' \tuple{\istr',\counter' \csep \wstrl',\cods{\elem}, 
   \wstrr' \csep \cods{\state} }
      \hfill\mbox{if $\state\in\Statesfin$}\\[3pt]
      
 S \counter' 
      \hfill\mbox{\qquad if 
      $\delta(\bool,\elem,\state)=(0 \csep \elem',\downarrow \csep \state')$}\\[3pt]
      
   L \counter' 
      \hfill \mbox{if 
      $\delta(\bool,\elem,\state)=(0\csep \elem',\leftarrow \csep \state')$}
      \\[3pt]
       
      
   R \counter' 
      \hfill \mbox{if 
      $\delta(\bool,\elem,\state)=(0\csep \elem',\rightarrow \csep \state')$}\\[3pt]
  
 \predl  S \counter'
  \hfill\mbox{\qquad if 
  	$\delta(\bool,\elem,\state)=(-1\csep \elem',\downarrow \csep \state')$}\\[3pt]
  
\predl L \counter'
  \hfill \mbox{if 
  	$\delta(\bool,\elem,\state)=(-1\csep \elem',\leftarrow \csep \state')$
	}
	\\[3pt]
  
  
  \predl R \counter'
  \hfill \mbox{if 
  	$\delta(\bool,\elem,\state)=(-1\csep \elem',\rightarrow \csep \state')$}

   \\[3pt]
   
   \succl S \counter'
  \hfill\mbox{\qquad if 
  	$\delta(\bool,\elem,\state)=(+1\csep \elem',\downarrow \csep \state')$}\\[3pt]
  
\succl L \counter'
  \hfill \mbox{if 
  	$\delta(\bool,\elem,\state)=(+1\csep \elem',\leftarrow \csep \state')$
	}
	\\[3pt]
  
  
  \succl  R \counter'
  \hfill \mbox{if 
  	$\delta(\bool,\elem,\state)=(+1\csep \elem',\rightarrow \csep \state')$}
   \end{array}
    \right.
    
    \\[3pt]
    S & \defeq & \la {\counter''} \var\cont' \tuple{\istr',\counter''\csep 
  	\wstrl',\cods{\elem'}, \wstrr' \csep \cods{\state'}} 
    \\
    L & \defeq & \la{\counter''}\wstrl' L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrr'
    \\
    R & \defeq & \la{\counter''}\wstrr' R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrl'
    \\
    L_{\elem''}^{\state',\elem'}
      & \defeq &
      \la{\wstrl'} \la\var \la{\cont'} \la{\istr'} \la{\counter'}\appendchar{\elem'}(\lambda \wstrr'.\var\cont' 
\tuple{\istr',\counter' \csep \wstrl',\cods{\elem''},\wstrr' \csep \cods{\state'}})
\\[3pt]
    L_{\ems}^{\state',\elem'}
      & \defeq &
\la\var \la{\cont'} \la{\istr'} \la{\counter'}
       \appendchar{\elem'}((\la d \lambda \wstrr'.\var\cont' 
      \tuple{\istr',\counter'\csep d,\cods{\elemblank},\wstrr' \csep  
      \cods{\state'}})\enc\ems)
      \\[3pt]
          R_{\elem''}^{\state',\elem'}
           & \defeq &
      \la{\wstrr'} \la\var \la{\cont'} \la{\istr'} \la{\counter'}\appendchar{\elem'}(\lambda \wstrl'.\var\cont' 
\tuple{\istr',\counter' \csep \wstrl',\cods{\elem''},\wstrr' \csep \cods{\state'}})
\\[3pt]
    R_{\ems}^{\state',\elem'}
      & \defeq &
\la\var \la{\cont'} \la{\istr'} \la{\counter'}
       \appendchar{\elem'}((\la d \lambda \wstrl'.\var\cont' 
      \tuple{\istr',\counter'\csep \wstrl',\cods{\elemblank},d \csep  
      \cods{\state'}})\enc\ems)

\end{array}\]

Let $C=(\istr,\counter \csep \wstrl,\elem,\wstrr \csep \state)$. We are now 
going to show the details of how the $\l$-calculus simulates the transition 
function. At the level of the number of steps, the main cost is payed at the 
beginning, by the $\lookupl$ function that looks up the $\counter$-th character 
of the input string $\istr$. The cost of one such call is 
$\bigo{\counter\log\counter}$, but since $n$ can vary and $n\leq \size\istr$, 
such a cost is bound by $\bigo{\size\istr\log{\size\istr}}$. The cases of 
transition where the position on the input tape does not change have a constant 
cost. Those where the input position changes require to change the counter 
$\counter$ via $\predl$ or $\succl$, which requires $\bigo{\log \counter}$, 
itself bound by the cost $\bigo{\size\istr\log{\size\istr}}$ of the previous 
look-up.

Now, if $\lookupf\, \ntostr n \istr = \bool$ then:
\begin{center}
$\begin{array}{llllll}
\transs\,  \cont\,  \enc\config & = & \fix \transaux \cont  \enc\config 
\\ & \tobdet^2 &
\transaux (  \la\varthree\fix \transaux\varthree ) \cont  \enc\config
\\ & = &
\transaux ( \la\varthree\transs\,\varthree  ) \cont  \enc\config
\\ & = &
(\lambda \var.\la{\cont'}\lambda \config'.\config'(\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K \istr' \counter')) ( \la\varthree\transs\,\varthree  ) \cont  \enc\config
\\ & \tobdet^3 &
\enc\config(\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K\isub\var{\la\varthree\transs\,\varthree} \istr' \counter')
\\ & = &
\enc{(\istr,\counter\csep \wstrl,\elem,\wstrr \csep \state)} (\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K\isub\var{\la\varthree\transs\,\varthree} \istr' \counter')
\\ & = &
(\lambda x. x\enc{\istr}\enc{\ntostr\counter}
\enc{\wstrl^\rop} \;\cods{\elem} \;\enc\wstrr \;\cods{\state} )
 (\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K\isub\var{\la\varthree\transs\,\varthree} \istr' \counter')

\\ & = &
(\la{\istr'}\la{\counter'}\la{\wstrl'}\la{\elem'}\la{\wstrr'}\la{\state'}\lookupl\,K\isub\var{\la\varthree\transs\,\varthree} \istr' \counter')
 \enc{\istr}\enc{\ntostr\counter}
\enc{\wstrl^\rop} \;\cods{\elem} \;\enc\wstrr \;\cods{\state} 


\\ & \tobdet^{6} &
\lookupl\,(\la {\bool'} \bool'\, 
A_{0}A_{1}A_{\stsym}A_{\ensym}\cods\elem\, \cods\state 
(\la\varthree\transs\,\varthree) \cont' \enc\istr \enc{\ntostr\counter} 
\enc{\wstrl^{\rop}} \enc{\wstrr}) \enc\istr \enc{\ntostr\counter}

 \\ \reflemmaeq{look} & \tobdet^{\bigo{\size\counter\log\size\counter}} &
 (\la {\bool'} \bool'\, 
A_{0}A_{1}A_{\stsym}A_{\ensym}\cods\elem\, \cods\state 
(\la\varthree\transs\,\varthree) \cont' \enc\istr \enc{\ntostr\counter} 
\enc{\wstrl^{\rop}} \enc{\wstrr}
)\cods\bool 

 \\ & \tobdet &
\cods\bool\, 
A_{0}A_{1}A_{\stsym}A_{\ensym} \cods{\elem}\, \cods{\state} ( 
\la\varthree\transs\,\varthree) \cont \enc{\istr}\enc{\ntostr\counter}
\enc{\wstrl^\rop}  \enc\wstrr

 \\ & \tobdet^{4} &
A_{\bool} \cods{\elem}\,\cods{\state} ( \la\varthree\transs\,\varthree) \cont \enc{\istr}\enc{\ntostr\counter}
\enc{\wstrl^\rop} \;\enc\wstrr 

 \\ & = &
(\la{\elem'} \elem' B_{\bool,0} B_{\bool,1} B_{\bool,\elemblank} ) \cods{\elem}\,\cods{\state} ( \la\varthree\transs\,\varthree) \cont \enc{\istr}\enc{\ntostr\counter}
\enc{\wstrl^\rop} \;\enc\wstrr 

 \\ & \tobdet &
 \cods\elem B_{\bool,0} B_{\bool,1} B_{\bool,\elemblank} \cods\state ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr

  \\ & \tobdet^{3} &
  B_{\bool,\elem} \cods\state ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr

    \\ & = &
  (\la{\state'}\state' C_{\bool,\elem,\state_{1}}\ldots C_{\bool,\elem,\state_{\size\States}}) \cods\state ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr

    \\ & \tobdet &
  \cods\state C_{\bool,\elem,\state_{1}}\ldots C_{\bool,\elem,\state_{\size\States}}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr

    \\ & \tobdet^{\size\States} &
    C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr

\end{array}$
 \end{center}
  
 Now, consider the following 
 four cases, depending on the value of $\delta(\bool,\elem,\state)$:
 \begin{enumerate}
   %%% CASE 1
    \item \emph{Final state}: 
    if $\delta(\bool,\elem,\state)$ is undefined, then $\state \in\Statesfin$ and replacing $C_{\bool,\elem,\state}$ with the corresponding $\l$-term we obtain:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
& = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} \cont' \tuple{\istr',\counter' \csep \wstrl',\cods{\elem}, \wstrr' \csep \cods{\state} }) ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
    \\
    & \tobdet^6 &
   \cont  \tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\wstrl^{\rop}} ,\cods{\elem}, \enc\wstrr \csep \cods{\state} }\\
    &=&\cont  \enc{(\istr,\counter \csep \wstrl ,\elem,\wstrr \csep \state)}\\
    &=&\cont  \enc\config\\
\end{array}$
\end{center}
 
    %%% CASE 2
    \item \emph{The heads do not move}: 
    if 
    $\delta(\bool,\elem,\state)=(0 \csep \elem',\downarrow \csep \state')$,
     then $\configtwo = (\istr,\counter \csep \wstrl, \elem',\wstrr,\state')$. The simulation continues as follows:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
        (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
S \counter')
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\    & = &
        (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
(\la{\counter''}\var\cont' \tuple{\istr',\counter''\csep 
   \wstrl',\cods{\elem'}, \wstrr' \csep \cods{\state'}}) \counter')
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
  (\la{\counter''}( \la\varthree\transs\,\varthree) \cont  \tuple{\enc\istr,\counter'' \csep \enc{\wstrl^{\rop}} ,\cods{\elem'}, \enc\wstrr \csep \cods{\state'} })\enc{\ntostr\counter}
\\   & \tobdet^{2} &
  \transs\, \cont  \tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\wstrl^{\rop}} ,\cods{\elem'}, \enc\wstrr \csep \cods{\state'} }
\\   & = &
  \transs\, \cont  \enc{(\istr,\counter \csep \wstrl , \elem', \wstrr \csep \state')}
\\   & = &
  \transs\, \cont  \enc{\configtwo}
\end{array}$
\end{center}

    %%% CASE 3
    \item \emph{The input head does not move and the work head moves left}: if 
      $\delta(\bool,\elem,\state)=(0\csep \elem',\leftarrow \csep \state')$ and $\wstrl = \wstr \elem''$ then:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
&&(\la\var \la{\cont'} \la{\istr'} \la{\counter''} \la{\wstrl'} \la{\wstrr'} 
L \counter') ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
 (\la{\counter''}\wstrl' L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrr') \counter')
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
(\la{\counter''}\enc{\wstrl^{\rop}}  L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc\wstrr)\enc{\ntostr\counter}
\\   & \tobdet &
\enc{\wstrl^{\rop}}  L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr
\end{array}$
\end{center}
      
    Two sub-cases, depending on whether $\wstrl$ is an empty or a compound string.
    
    \begin{enumerate}
    %%% CASE 3.1
	 \item \emph{$\wstrl$ is the compound string $\wstr\elem''$}. Then $\wstrl^{\rop} = \elem'' \wstr^{\rop}$ and $\configtwo = (\istr,\counter \csep \wstrl, \elem'',\elem'\wstrr \csep \state')$. The simulation continues as follows:
    \begin{center}
$\begin{array}{llllll}
   & = &
\enc{\elem''\wstr^{\rop}}  L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr

\\   & \tobdet^{4} &
  L_{\elem''}^{\state',\elem'} \enc{\wstr^{\rop}}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr
\\   & = &  
        (\la{\wstrl'} \la\var \la{\cont'} \la{\istr'} \la{\counter'}\appendchar{\elem'}(\lambda \wstrr'.\var\cont' 
\tuple{\istr',\counter' \csep \wstrl',\cods{\elem''},\wstrr' \csep \cods{\state'}}))
\enc{\wstr^{\rop}}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr
\\   & \tobdet^{5} &  
        \appendchar{\elem'}(\lambda \wstrr'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\wstr^{\rop}},\cods{\elem''},\wstrr' \csep \cods{\state'}})
 \enc\wstrr
 
\\ \reflemmaeq{append-char}    & \tobdet^{ O(1) } & 
(\lambda \wstrr'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\wstr^{\rop}},\cods{\elem''},\wstrr' \csep \cods{\state'}})
 \enc{\elem'\wstrr}
\\    & \tobdet^{2} & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\wstr^{\rop}},\cods{\elem''}, \enc{\elem'\wstrr} \csep \cods{\state'}}
\\    & = & 
\transs\, \cont 
\enc{(\istr,\counter \csep \wstr,\elem'', \elem'\wstrr \csep \state')}
\\    & = & 
\transs\, \cont \enc{\configtwo}
\end{array}$
\end{center}
    
    	 \item \emph{$\wstrl$ is the empty string $\varepsilon$}. Then $\configtwo = (\istr,\counter \csep \ems, \elemblank,\elem'\wstrr \csep \state')$. The simulation continues as follows:
    \begin{center}
$\begin{array}{llllll}
   & = &
\enc{\ems}  L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'}   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr

\\   & \tobdet^{4} &
  L_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr
\\   & = &  
        ( \la\var \la{\cont'} \la{\istr'} \la{\counter'}
       \appendchar{\elem'}((\la d \lambda \wstrr.\var\cont' 
      \tuple{\istr',\counter'\csep d,\cods{\elemblank},\wstrr \csep  
      \cods{\state'}})\enc\ems))
 ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc\wstrr
\\   & \tobdet^{5} &  
        \appendchar{\elem'}((\la d \lambda \wstrr'. ( 
        \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep d,\cods{\elemblank},\wstrr' \csep 
\cods{\state'}})\enc\ems)
 \enc\wstrr
 
\\ \reflemmaeq{append-char}    & \tobdet^{ O(1) } & 
((\la d \lambda \wstrr'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep d,\cods{\elemblank},\wstrr' \csep 
\cods{\state'}})\enc\ems)
 \enc{\elem'\wstrr}
\\    & \tobdet^{3} & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc\ems,\cods{\elemblank}, 
\enc{\elem'\wstrr} \csep \cods{\state'}}
\\    & = & 
\transs\, \cont 
\enc{(\istr,\counter \csep \ems,\elemblank, \elem'\wstrr \csep \state')}
\\    & = & 
\transs\, \cont \enc{\configtwo}
\end{array}$
\end{center}
\end{enumerate}
  
  %%% CASE 4
    \item \emph{The input head does not move and the work head moves right}:  if 
      $\delta(\bool,\elem,\state)=(0\csep \elem',\rightarrow \csep \state')$ and $\wstrr = \elem'' \wstr $ then:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
 R \counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
 (\la{\counter''}\wstrr' R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrl') \counter')
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
(\la{\counter''}\enc{\wstrr}  R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc{\wstrl^{\rop}})\enc{\ntostr\counter}
\\      & \tobdet &
\enc{\wstrr}  R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\end{array}$
\end{center}
      
    Two sub-cases, depending on whether $\wstrl$ is an empty or a compound string.
    
    \begin{enumerate}
    %%% CASE 3.1
	 \item \emph{$\wstrr$ is the compound string $\elem''\wstr$}. Then  $\configtwo = (\istr,\counter \csep \wstrl\elem', \elem'',\wstr \csep \state')$. The simulation continues as follows:
    \begin{center}
$\begin{array}{llllll}
   & = &
\enc{\elem''\wstr}  R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}

\\   & \tobdet^{4} &
  R_{\elem''}^{\state',\elem'} \enc{\wstr}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\\   & = &  
        (\la{\wstrr'} \la\var \la{\cont'} \la{\istr'} \la{\counter'}\appendchar{\elem'}(\lambda \wstrl'.\var\cont' 
\tuple{\istr',\counter' \csep \wstrl',\cods{\elem''},\wstrr' \csep \cods{\state'}}))
\enc{\wstr}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\\   & \tobdet^{5} &  
        \appendchar{\elem'}(\lambda \wstrl'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \wstrl',\cods{\elem''},\wstr \csep \cods{\state'}})
 \enc{\wstrl^{\rop}}
 
\\ \reflemmaeq{append-char}    & \tobdet^{ O(1) } & 
(\lambda \wstrl'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \wstrl',\cods{\elem''},\wstr \csep \cods{\state'}})
 \enc{\elem'\wstrl^{\rop}}
\\    & \tobdet^{2} & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep  \enc{\elem'\wstrl^{\rop}},\cods{\elem''},\wstr \csep \cods{\state'}}
\\    & = & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep  \enc{(\wstrl\elem')^{\rop}},\cods{\elem''},\wstr \csep \cods{\state'}}
\\    & = & 
\transs\, \cont 
\enc{(\istr,\counter \csep \wstrl\elem',\elem'', \wstr \csep \state')}
\\    & = & 
\transs\, \cont \enc{\configtwo}
\end{array}$
\end{center}
    
    	 \item \emph{$\wstrr$ is the empty string $\varepsilon$}. Then $\configtwo = (\istr,\counter \csep \wstrl\elem', \elemblank,\ems \csep \state')$. The simulation continues as follows:
    \begin{center}
$\begin{array}{llllll}
   & = &
\enc{\ems}  R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\\   & \tobdet^{4} &
  R_{\ems}^{\state',\elem'}  ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\\   & = &  
        (\la\var \la{\cont'} \la{\istr'} \la{\counter'}
       \appendchar{\elem'}((\la d \lambda \wstrl'.\var\cont' 
      \tuple{\istr',\counter'\csep \wstrl',\cods{\elemblank},d \csep  
      \cods{\state'}})\enc\ems)
)
 ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}}
\\   & \tobdet^{5} &  
        \appendchar{\elem'}((\la d \lambda \wstrl'. ( 
        \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \wstrl',\cods{\elemblank},d \csep 
\cods{\state'}})\enc\ems)
\enc{\wstrl^{\rop}}
 
\\ \reflemmaeq{append-char}    & \tobdet^{ O(1) } & 
((\la d \lambda \wstrl'. ( \la\varthree\transs\,\varthree) \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \wstrl',\cods{\elemblank},d \csep 
\cods{\state'}})\enc\ems)
 \enc{\elem'\wstrl^{\rop}}
\\    & \tobdet^{3} & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{\elem'\wstrl^{\rop}},\cods{\elemblank}, \enc{\ems} \csep \cods{\state'}})
\\    & = & 
\transs\, \cont 
\tuple{\enc\istr,\enc{\ntostr\counter} \csep \enc{(\wstrl\elem')^{\rop}},\cods{\elemblank}, \enc{\ems} \csep \cods{\state'}})
\\    & = & 
\transs\, \cont 
\enc{(\istr,\counter \csep \wstrl\elem',\elemblank, \ems \csep \state')}
\\    & = & 
\transs\, \cont \enc{\configtwo}
\end{array}$
\end{center}
\end{enumerate}

%%% CASE 5
    \item \emph{The input head moves left and the work head does not move}: 
    if 
    $\delta(\bool,\elem,\state)=(-1 \csep \elem',\downarrow \csep \state')$,
     then $\configtwo = (\istr,\counter-1 \csep \wstrl, \elem',\wstrr,\state')$. The simulation continues as follows:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl\, S 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
   \\ & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl\, (\la {\counter''} x\cont' \tuple{\istr',\counter''\csep 
  	\wstrl',\cods{\elem'}, \wstrr' \csep \cods{\state'}} )\counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
  \predl\, (\la {\counter''} ( \la\varthree\transs\,\varthree)\cont \tuple{\enc\istr,\counter''\csep 
  	\enc{\wstrl^{\rop}},\cods{\elem'}, \enc\wstrr \csep \cods{\state'}} )\enc{\ntostr\counter}
\\  \reflemmaeq{pred} & \tobdet^{\bigo{\log n}} &
(\la {\counter''} ( \la\varthree\transs\,\varthree)\cont \tuple{\enc\istr,\counter''\csep 
  	\enc{\wstrl^{\rop}},\cods{\elem'}, \enc\wstrr \csep \cods{\state'}} )\enc{\ntostr{\counter-1}}
	\\   & = &
  \transs\, \cont  \enc{(\istr,\ntostr{\counter-1} \csep \wstrl , \elem', \wstrr \csep \state')}
  \\   & = &
  \transs\, \cont  \enc{(\istr,\ntostr{\counter-1} \csep \wstrl , \elem', \wstrr \csep \state')}
\\   & = &
  \transs\, \cont  \enc{\configtwo}
\end{array}$
\end{center}


%%% CASE 6
    \item \emph{The input head moves left and the work head moves left}: 
    if 
    $\delta(\bool,\elem,\state)=(-1 \csep \elem',\leftarrow \csep \state')$ and $\wstrl = \wstr\elem''$,
     then $\configtwo = (\istr,\counter-1 \csep \wstr, \elem'', \elem'\wstrr,\state')$. The simulation continues as follows:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl\, L \counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl\, (\la{\counter''}\wstrl' L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrr')\counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
  \predl\, (\la{\counter''}\enc{\wstrl^{\rop}} L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc\wstrr)\enc{\ntostr\counter}
  
\\  \reflemmaeq{pred} & \tobdet^{\bigo{\log n}} &
(\la{\counter''}\enc{\wstrl^{\rop}} L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc\wstrr)
\enc{\ntostr{\counter-1}}
	\\   & \tobdet &
  \enc{\wstrl^{\rop}} L_0^{\state',\elem'} L_1^{\state',\elem'} L_{\elemblank}^{\state',\elem'}L_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr{\counter-1}} \enc\wstrr
\end{array}$
\end{center}
And then the case continues with the two sub-cases of case 3 (input head does not move and work head moves left), with the only difference that $\enc{\ntostr{\counter}}$ is replaced by $\enc{\ntostr{\counter-1}}$.

%%% CASE 7
    \item \emph{The input head moves left and the work head moves right}: 
    if 
    $\delta(\bool,\elem,\state)=(-1 \csep \elem',\leftarrow \csep \state')$ and $\wstrl = \wstr\elem''$,
     then $\configtwo = (\istr,\counter-1 \csep \wstr, \elem'', \elem'\wstrr,\state')$. The simulation continues as follows:
\begin{center}
$\begin{array}{llllll}
&&C_{\bool,\elem,\state} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl\, R \counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\	
    & = &
    (\la\var \la{\cont'} \la{\istr'} \la{\counter'} \la{\wstrl'} \la{\wstrr'} 
\predl (\la{\counter''}\wstrr' R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} \var \cont' \istr' \counter'' \wstrl'
)\counter') 
   ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr\counter} \enc{\wstrl^{\rop}} \enc\wstrr
\\   & \tobdet^{6} &
  \predl (\la{\counter''}\enc{\wstrr} R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc{\wstrl^{\rop}})\enc{\ntostr\counter}
  
\\  \reflemmaeq{pred} & \tobdet^{\bigo{\log n}} &
(\la{\counter''}\enc{\wstrr} R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \counter'' \enc{\wstrl^{\rop}})
\enc{\ntostr{\counter-1}}
	\\   & \tobdet &
  \la{\counter''}\enc{\wstrr} R_0^{\state',\elem'} R_1^{\state',\elem'} R_{\elemblank}^{\state',\elem'}R_{\ems}^{\state',\elem'} ( \la\varthree\transs\,\varthree) \cont \enc\istr \enc{\ntostr{\counter-1}} \enc{\wstrl^{\rop}}
\end{array}$
\end{center}
And then the case continues with the two sub-cases of case 4 (input head does not move and work head moves right), with the only difference that $\enc{\ntostr{\counter}}$ is replaced by $\enc{\ntostr{\counter-1}}$.

\item \emph{The input head moves right and the work head does not move}: exactly as case 5 (input head \emph{left}, work head does not move) just replacing $\predl$ with $\succl$ and using \reflemma{succ} instead of \reflemma{pred}.

\item \emph{The input head moves right and the work head moves left}: exactly as case 6 (input head \emph{left}, work head left) just replacing $\predl$ with $\succl$ and using \reflemma{succ} instead of \reflemma{pred}.

\item \emph{The input head moves right and the work head moves right}: exactly as case 7 (input head \emph{right}, work head right) just replacing $\predl$ with $\succl$ and using \reflemma{succ} instead of \reflemma{pred}.
\end{enumerate}


==> proofs/preliminaries/lookup-proof.tex <==
% !TEX root = ../../main.tex
\begin{proof}

We can now code the function $\lookupl \defeq \fix \lookupaux$ where:
\[
\lookupaux \defeq \la\varf{\la {\cont'}{\la {\counter'}{\la {\inputstr'}{\counter'N_{0}N_{1}N_\ems \varf \cont' \inputstr'}}}}
\]
where:
\begin{itemize}
	\item $N_{0}\defeq \la{\strthree'}\la\varf\la{\cont'}\la{\inputstr'}\inputstr' M_{0} 
	M_{0} M_\ems \strthree' \varf \cont' $, where
	\begin{itemize}
	\item $M_{0}\defeq \la{\strtwo'}\la{\strthree'}\la\varf\la{\cont'} \appendchar0  (\la{\varthree''}\predl(\la{\varthree'}\varf\cont'\varthree' ) \varthree'') \strthree' \strtwo'$;
	\item $M_\ems$ is whatever closed term.
	\end{itemize}
	
	\item $N_{1}\defeq \la{\strthree'}\la\varf\la{\cont'}\la{\inputstr'}\inputstr' M_{1} M_{1} M_\ems  \strthree' \varf \cont'$, where
	\begin{itemize}
	\item $M_{1}\defeq \la{\strtwo'}\la{\strthree'}\la\varf\la{\cont'} \appendchar1  (\la{\varthree''}\predl(\la{\varthree'}\varf\cont'\varthree' ) \varthree'') \strthree' \strtwo'$;
	\item $M_\ems$ is whatever closed term.
	\end{itemize}
	
	\item $N_\ems\defeq \la\varf\la{\cont'}\la{\inputstr'}\inputstr' O_0 O_{1} 
	O_\stsym O_\ensym O_{\ems} \cont'$, where 
	
	\begin{itemize}
	\item $O_\bool \defeq \la{\str'}\la {\cont'} \cont' \cods{\bool}$;
	\item $O_\ems$ is whatever closed term.
	\end{itemize}
\end{itemize}
The first steps of the evaluation of $\lookupl\,\cont\enc{\ntostr \counter}\enc{\inputstr}$ are common to all strings $\inputstr\in\Bool^+$ and natural numbers $\counter\in\nat$:
\[\begin{array}{llllllll}
\lookupl\,\cont\enc{\ntostr \counter}\enc{\inputstr} & = & \fix \lookupaux\, k\enc{\ntostr \counter}\enc{\inputstr}
\\ & \tob^{2} &
\lookupaux (\la\varthree \lookupl\, \varthree) \cont\enc{\ntostr \counter}\enc{\inputstr}
\\ & = &
(\la\varf{\la {\cont'}{\la {\counter'}{\la {\inputstr'}{\counter'N_{0}N_{1}N_\ems \varf \cont' \inputstr'}}}}) (\la\varthree \lookupl\,\varthree)  \cont\enc{\ntostr \counter}\enc{\inputstr}
\\ & \tob^{4} &
\enc{\ntostr \counter} N_{0} N_{1} N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc{\inputstr}
\end{array}\]
Cases of $n$:
\begin{itemize}
\item $n=0$, and so $\ntostr \counter = \ems$: then  
\[\begin{array}{llllllll}
&&\enc{\ems} N_{0}N_{1} N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) N_{0}N_{1} N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & \tob^{3} &
N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & = &
(\la\varf\la{\cont'}\la{\inputstr'}\inputstr' O_0 O_{1} O_\stsym O_\ensym 
O_{\ems} \cont') (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & \tobdet^{3} &
\enc\inputstr O_0 O_{1} O_\stsym O_\ensym O_{\ems} \cont
\end{array}\]
Let $\inputstr$ start with $\bool\in \Bool$, that is, $\inputstr = \bool\cons\str$:
\[\begin{array}{llllllll}
\enc{\bool\cons\str}\, O_0 O_{1} O_\stsym O_\ensym O_{\ems} \cont
& = & 
(\la{\var_{0}}\la{\var_{1}}\la\var_{\ems}\var_{\bool} \enc\str) O_{0} O_{1} 
O_\stsym O_\ensym O_{\ems} \cont
\\ & \tobdet^{3} &
O_{\bool} \enc\str \cont
\\ & = &
(\la{\str'}\la {\cont'} \cont'\cods{\bool}) \enc\str \cont
\\ & \tob^{2} &
\cont \cods{\bool} 
\\ & = & 
\cont \cods{\lookupf\, \ems (\bool\cons\str)}
\\ & = & 
\cont \cods{\lookupf\, \ntostr 0 \istr}
\end{array}\]

\item \emph{Non-empty string starting with $0$}, that is, $n>0$ and $\ntostr \counter = 0 \cons \strthree$: then  
\[\begin{array}{llllllll}
&&\enc{\ntostr \counter} N_{0}N_{1}N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo \var_{0} \enc{\strthree}}}) N_{0}N_{1}N_{\ems} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & \tob^{3} &
N_{0} \enc{\strthree} (\la\varthree \lookupl\,\varthree) \cont \enc\inputstr
\\ & = &
( \la{\strthree'}\la\varf\la{\cont'}\la{\inputstr'}\inputstr' M_{0} 
	M_{0} M_\ems \strthree' \varf \cont' )\enc{\strthree} (\la\varthree \lookupl\,\varthree)\cont \enc\inputstr
\\ & \tob^{4} &
\enc\inputstr M_{0} M_{0} M_\ems \enc{\strthree} (\la\varthree \lookupl\,\varthree) \cont
\end{array}\]
Let $\inputstr$ start with $\bool\in \Bool$, that is, $\inputstr = \bool\cons\strtwo$:

%\begin{itemize}
%\item $\str$ is empty:
%\[\begin{array}{llllllll}
%\enc\ems M'M' M_\ems \cont
%& = & 
%(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) M'M' M_\ems \cont
%\\ & \tobdet^{3} &
%M_\ems \cont
%\\ & = &
%(\la y y\cods{0}) \cont
%\\ & \tob &
%\cont \cods{0} 
%\\ & = & 
%\cont (\cods{\lookupf\, \ntostr \counter \ems})
%\end{array}\]

%\item 
\[\begin{array}{llllllll}
\enc{\bool\cons\strtwo} M_{0} M_{0} M_\ems \cont
& = & 
(\la{\var_{0}}\la{\var_{1}}\la{\var_{\ems}} \var_{\bool} \enc\strtwo) M_{0} M_{0} M_\ems \enc{\strthree} (\la\varthree \lookupl\,\varthree) \cont
\\ & \tobdet^{\size\alpone} &
M_{0} \enc\strtwo\, \enc{\strthree} (\la\varthree \lookupl\,\varthree) \cont
\\ & = &
(\la{\strtwo'}\la{\strthree'}\la\varf\la{\cont'} \appendchar0  (\la{\varthree''}\predl(\la{\varthree'}\varf\cont'\varthree' ) \varthree'') \strthree' \strtwo') \enc\strtwo\, \enc{\strthree} (\la\varthree \lookupl\,\varthree)\cont
\\ & \tobdet^{4} &
\appendchar0  (\la{\varthree''}\predl(\la{\varthree'}(\la\varthree \lookupl\,\varthree)\cont\varthree' ) \varthree'')  \enc\strthree\, \enc\strtwo
\\ (\reflemmaeq{append-char} & \tobdet^{\bigo{1}} &
(\la{\varthree''}\predl(\la{\varthree'}(\la\varthree \lookupl\,\varthree)\cont\varthree' ) \varthree'') \enc{0\cons\strthree}\, \enc\strtwo
\\ & \tobdet &
\predl(\la{\varthree'}(\la\varthree \lookupl\,\varthree)\cont\varthree' ) \enc{0\cons\strthree}\, \enc\strtwo
\\ & = &
\predl(\la{\varthree'}(\la\varthree \lookupl\,\varthree)\cont\varthree' ) \enc{\ntostr \counter}\, \enc\strtwo
\\ (\reflemmaeq{pred}) & \tobdet^{\bigo{\size{\ntostr \counter}}} &
(\la{\varthree'}(\la\varthree \lookupl\,\varthree)\cont\varthree' ) \enc{\predf\, \ntostr \counter}\, \enc\strtwo
\\ & \tobdet^{2} &
\lookupl\, \cont\, \enc{\predf\,\ntostr \counter}\, \enc\strtwo
\\ & = &
\lookupl\, \cont\, \enc{\ntostr{ n-1}}\, \enc\strtwo
\\ (\ih) & \tobdet^{\bigo{(n-1)\cdot\log{(n-1)}}} &
\cont (\cods{\lookupf\, \ntostr{n-1} \strtwo})
\\
\\ & = & 
\cont (\cods{\lookupf\, \ntostr \counter \str})
\end{array}\]

The number of $\beta$ steps then is $\bigo{\size{\ntostr \counter}} + \bigo{(\counter-1)\cdot\log{(\counter-1)}} + h$ for a certain constant $h$. Since $\size{\ntostr \counter} = \bigo{\log \counter}$, we obtain that the number of steps is bound by $\bigo{\counter\cdot\log{\counter}}$, as required.
%\end{itemize}

\item \emph{Non-empty string starting with $1$}, that is, $n>0$ and $\ntostr \counter = 1 \cons \strthree$: same as the previous one, simply replacing $N_{0}$ with $N_{1}$, and thus $M_{0}$ with $M_{1}$. In particular, it takes the same number of steps.
\end{itemize}
\end{proof}

==> proofs/preliminaries/pred-proof.tex <==
% !TEX root = ../../main.tex
\begin{proof}
Define 
$\predl \defeq \fix\predaux$ and $\predaux \defeq \la\varf{\la {\cont'}{\la {\counter'}{\counter' N_0N_1N_\ems \varf\cont'}}}$ 
where:
\begin{itemize}
	\item $N_0\defeq \la {\strtwo'}\la\varf\la {\cont'}{\varf(\la\varthree\appendchar1\cont'\varthree)\strtwo'}$;
	\item $N_1\defeq \la {\strtwo'}\la\varf{{\strtwo'}M_{0}M_{1}M_\ems}$, where:
	\begin{itemize}
	\item $M_0\defeq \la v{\la k{\appendchar0(\la\varthree\appendchar1\cont\varthree) v}}$;
	\item $M_1\defeq \la v{\la k{\appendchar1(\la\varthree\appendchar1\cont\varthree) v}}$;
	\item $M_\ems\defeq \la {\cont'} \cont'\enc\ems$;
\end{itemize}

	\item $N_{\ems}$ is whatever closed term.
\end{itemize}
The first steps of the evaluation of $\predl\, \cont \enc{\ntostr\counter}$ are common to all natural numbers $1\leq \counter\in\nat$:
\[\begin{array}{llllllll}
\predl\, \cont \enc{\ntostr\counter} & = & \fix \predaux\, \cont \enc{\ntostr\counter}
\\ & \tob^{2} &
\predaux (\la\varthree \predl\, \varthree) \cont \enc{\ntostr\counter}
\\ & = &
(\la\varf{\la {\cont'}{\la {\counter'}{\counter' N_0N_1N_\ems \varf\cont'}}}) (\la\varthree \predl\, \varthree) \cont \enc{\ntostr\counter}
\\ & \tob^{3} &
\enc{\ntostr\counter} N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
\end{array}\]

By hypothesis, $\counter\geq 1$. Then $\enc\counter$ is a non-empty string. Cases of its first character:
\begin{itemize}
%\item \emph{Zero}, that is, $\counter =0 $, $\ntostr\counter = \ems$, and $\enc{\ntostr\counter} = \la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}$: then  
%\[\begin{array}{llllllll}
%\enc{\ntostr\counter} N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
%& = & 
%(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
%\\ & \tob^{3} &
%N_{\ems} (\la\varthree \predl\, \varthree) \cont
%\\ & = &
%(\la\varf \la {\cont'} \cont' \enc{1\cons\ems}) (\la\varthree \predl\, \varthree) \cont
%\\
% & \tob^{2} & 
% \cont \enc{1\cons\ems}
% \\ & = &  \cont \enc{\predf\, {\ntostr\counter}}
%\end{array}\]

\item \emph{$0$ character}, \ie ${\ntostr\counter} = 0\cons\strtwo$: then 
\[\begin{array}{rlllllll}
\enc{\ntostr\counter} N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_0\enc{\strtwo}}}) N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
\\ 
& \tob^{3} &
N_0 \enc{\strtwo} (\la\varthree \predl\, \varthree) \cont
\\ & = &
(\la {\strtwo'}\la\varf\la {\cont'}{\varf(\la\varthree\appendchar1\cont'\varthree)\strtwo'}) \enc{\strtwo} (\la\varthree \predl\, \varthree) \cont
\\ & \tob^{3} & 
(\la\varthree \predl\, \varthree) (\la\varthree\appendchar1\cont'\varthree) \enc{\strtwo}
\\ & \tob & 
\predl (\la\varthree\appendchar1\cont\varthree) \enc{\strtwo}
\\ (\ih) & \tob^{\bigo{\size\strtwo}} &  
(\la\varthree\appendchar1\cont\varthree)\, \enc{\predf\, \strtwo}
\\  & \tob &  
\appendchar1\cont\, \enc{\predf\, \strtwo}
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  
\cont\, \enc{1\cons (\predf\, \strtwo)}
\\ & = &  \cont\, \enc{\predf\, {0\cons\strtwo}}
\\ & = &  \cont\, \enc{\predf\, {\ntostr\counter}}
\end{array}\]

\item \emph{$1$ character}, \ie ${\ntostr\counter} = 1\cons\strtwo$: then 
\[\begin{array}{rlllllll}
\enc{\ntostr\counter} N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_1\enc{\strtwo}}}) N_0 N_1N_\ems (\la\varthree \predl\, \varthree) \cont 
\\ 
& \tob^{3} &
N_1 \enc{\strtwo} (\la\varthree \predl\, \varthree) \cont
	\\ & = &
	(\la {\strtwo'}\la\varf{{\strtwo'}M_{0}M_{1}M_\ems})\enc{\strtwo} (\la\varthree \predl\, \varthree) \cont\\
	&\tob& \enc{\strtwo}M_0M_1M_\ems \cont
	\end{array}\]
	
	There are three sub-cases, depending on the string $\strtwo$:
	\begin{itemize}
	\item $\strtwo$ is empty, \ie $\strtwo=\ems$. Then:
	\[\begin{array}{rlllllll}
	\enc{\ems}M_0M_1M_\ems \cont &=&
	(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}})M_0M_1M_\ems k\\
	&\tob^3&M_\ems k
	\\ & = & 
	(\la {\cont'} \cont'\enc\ems)\cont
	\\  & \tob &  \cont \enc{ \ems}
		\\  & \tob &  \cont \enc{ \ntostr 0}
	\\ & = &  \cont \enc{\predf\, {\ntostr 1}}
\end{array}\]

\item \emph{$\strtwo$ start with $0$}, that is, 
$\ntostr\counter=1\cons\strtwo= 1\cons0\cons\strthree$. Then:
\[\begin{array}{rlllllll}
\enc{0\cons\strthree}\,M_0M_1M_\ems k&=&
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_{0}\enc\strthree}})M_0M_1M_\ems k\\
&\tob^3&M_0 \enc\strthree k
\\
&=&(\la v{\la k{\appendchar0(\la\varthree\appendchar0\cont\varthree) v}})\enc\strthree k
\\&\tob^2&
\appendchar0 (\la\varthree\appendchar0\cont\varthree) \enc\strthree
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  (\la\varthree\appendchar0\cont\varthree) \enc{ 0\cons\strthree}
\\ & \tob &  \appendchar0\cont\, \enc{ 0\cons\strthree}
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  
\cont\, \enc{0\cons0\cons\strthree}
\\ & = &  \cont\, \enc{0\cons\strtwo}
\\ & = &  \cont\, \enc{\predf\, {1\cons\strtwo}}
\\ & = &  \cont\, \enc{\predf\, {\ntostr\counter}}
\end{array}\]

\item \emph{$\strtwo$ start with $1$}, that is, 
$\ntostr\counter=1\cons\strtwo= 1\cons1\cons\strthree$. Then:
\[\begin{array}{rlllllll}
\enc{0\cons\strthree}\,M_0M_1M_\ems k&=&
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_{1}\enc\strthree}})M_0M_1M_\ems k\\
&\tob^3&M_1 \enc\strthree k
\\
&=&(\la v{\la k{\appendchar1(\la\varthree\appendchar0\cont\varthree) v}})\enc\strthree k
\\&\tob^2&
\appendchar1 (\la\varthree\appendchar0\cont\varthree) \enc\strthree
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  (\la\varthree\appendchar0\cont\varthree) \enc{ 1\cons\strthree}
\\ & \tob &  \appendchar0\cont\, \enc{ 1\cons\strthree}
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  
\cont\, \enc{0\cons1\cons\strthree}
\\ & = &  \cont\, \enc{0\cons\strtwo}
\\ & = &  \cont\, \enc{\predf\, {1\cons\strtwo}}
\\ & = &  \cont\, \enc{\predf\, {\ntostr\counter}}
\end{array}\]

\end{itemize}
\end{itemize}
\end{proof}

==> proofs/preliminaries/succ-proof.tex <==
% !TEX root = ../../main.tex
\begin{proof}
Define 
$\succl \defeq \Theta\succaux$ and
$\succaux \defeq \la\varf{\la {\cont'}{\la {\counter'}{\counter'N_0N_1N_{\ems} \varf \cont'}}}$
where:
\begin{itemize}
	\item $N_0\defeq \la{\varf'}\la {\str'}{\la {\cont'}{\appendchar1\cont' \str'}}$
	\item $N_1\defeq \la{\varf'}\la {\str'}{\la {\cont'}{\varf'(\la\varthree\appendchar0\cont' \varthree) \str'}}$
	\item $N_{\ems}\defeq \la{\varf'}\la {\cont'} \cont'\, \enc{1\cons\ems}$
\end{itemize}
The first steps of the evaluation of $\succl\, k \enc{\ntostr\counter}$ are common to all natural numbers $\counter\in\nat$:
\[\begin{array}{llllllll}
\succl\, \cont \enc{\ntostr\counter} & = & \fix \succaux\, \cont \enc{\ntostr\counter}
\\ & \tob^{2} &
\succaux (\la\varthree \succl\, \varthree) \cont \enc{\ntostr\counter}
\\ & = &
(\la\varf{\la {\cont'}{\la {\counter'}{\counter'N_0N_1N_{\ems} \varf \cont'}}}) (\la\varthree \succl\,\varthree) \cont \enc{\ntostr\counter}
\\ & \tob^{3} &
\enc{\ntostr\counter} N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
\end{array}\]

Cases of $\counter$:
\begin{itemize}
\item \emph{Zero}, that is, $\counter =0 $, $\ntostr\counter = \ems$, and $\enc{\ntostr\counter} = \la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}$: then  
\[\begin{array}{llllllll}
\enc{\ntostr\counter} N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont \\ & \tob^{3} &
N_{\ems} (\la\varthree \succl\,\varthree) \cont
\\ & = &
(\la{\varf'} \la {\cont'} \cont'\,\enc{1\cons\ems}) \cont
\\
 & \tob & \cont\, \enc{1\cons\ems}
 \\ & = &  \cont\, \enc{\succf\, \ntostr 0}
\end{array}\]

\item \emph{Not zero}. Then there are two sub-cases, depending on the first character of the string $\ntostr\counter$:
\begin{itemize}
\item \emph{$0$ character}, \ie $\ntostr\counter = 0\cons\str$: then 
\[\begin{array}{rlllllll}
\enc{0\cons\strtwo} N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_0\enc{\str}}}) N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
\\ & \tob^{3} &
N_{0} \enc{\str} (\la\varthree \succl\,\varthree) \cont 
\\ & = &
(\la{\varf'}\la {\str'}{\la {\cont'}{\appendchar1\cont' \str'}}) \enc{\str} (\la\varthree \succl\,\varthree) \cont 
\\ & \tob^{3} & 
 \appendchar1\cont \enc{\str}
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  
\cont\, \enc{1\cons\str}
\\ & = &  \cont\, \enc{\succf\, \ntostr\counter}
\end{array}\]

\item \emph{$1$ character}, \ie $\ntostr\counter = 1\cons\str$: then 
\[\begin{array}{rlllllll}
\enc{1\cons\strtwo} N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_1\enc{\str}}}) N_0N_1N_{\ems} (\la\varthree \succl\,\varthree) \cont 
\\ & \tob^{3} &
N_{1} \enc{\str} (\la\varthree \succl\,\varthree) \cont 
\\ & = &
(\la{\varf'}\la {\str'}{\la {\cont'}{\varf'(\la\varthree\appendchar0\cont'\varthree) \str'}}) \enc{\str} (\la\varthree \succl\,\varthree) \cont 
\\ & \tob^{3} & 
(\la\varthree \succl\,\varthree)\,(\la\varthree\appendchar0\cont\varthree)\enc{\str}
\\ & \tob & 
 \succl\,(\la\varthree\appendchar0\cont\varthree)\enc{\str}
\\ (\ih) & \tob^{\bigo{\size\str}} &  
(\la\varthree\appendchar0\cont\varthree)\enc{\succf\,\str}
\\ & \tobdet &
\appendchar0\cont \enc{\succf\,\str}
\\ (\reflemmaeq{append-char}) & \tob^{\bigo{1}} &  \cont\, \enc{ 0\cons(\succf\,\str)}
\\ & = &  \cont\, \enc{\succf\, (1\cons\str)}
\\ & = &  \cont\, \enc{\succf\, \ntostr\counter}
\end{array}\]
\end{itemize}
\end{itemize}
\end{proof}

==> proofs/preliminaries/write-proof.tex <==
% !TEX root = ../main.tex
\begin{proof}
We can now code the function $\writel \defeq \fix \writeaux$ where:
\[
\writeaux \defeq \la\var{\la k{\la n{\la \elem \la \strtwo{nNNN_\ems k}}}}
\]
where:
\begin{itemize}
	\item $N\defeq \la\varthree \strtwo M_{0}M_{1}M_{\elemblank} M_\ems$, where
	\begin{itemize}
	\item $M\defeq \la u{\la\cont{\predl(\var\cont )n u}}$\qquad\text{ forse da fare con append}
	\item $M_\ems\defeq\la y y\enc{\ems}$
	\end{itemize}
	
	\item $N_\ems\defeq \strtwo O_0 O_{1} O_{\elemblank} O_{\ems}$, where
	\begin{itemize}
	\item $O_0 \defeq \la\varthree \la y y\cods{0}$
	\item $O_1 \defeq \la\varthree \la y y\cods{1}$
	\item $O_1 \defeq \la\strtwo \la \cont \strtwo PPPP_{\ems} \cont$, where
	\begin{itemize}
		\item $P \defeq \ben{\ldots}$
		\item $P_{\ems} \defeq \la \vartwo \vartwo \enc{\elem\cons\elemblank\cons\ems}$
	\end{itemize}
	\item $O_\ems \defeq \la y y\cods{0}$
	\end{itemize}
\end{itemize}
The first steps of the evaluation of $\writel\,k\,\enc{\ntostr n}\, \enc\elem\, \enc{\str}$ are common to all characters $\elem\in\alponeblank$, strings $\str\in\alponeblank^*$, and natural numbers $n\in\nat$:
\[\begin{array}{llllllll}
\writel\,k\,\enc{\ntostr n}\, \enc\elem\, \enc{\str}& = & \fix \writeaux\, k\enc{\ntostr n}\enc{\str}
\\ & \tob^{2} &
\writeaux (\la\varthree \writel\, \varthree) k\,\enc{\ntostr n}\, \enc\elem\, \enc{\str}
\\ & = &
(\la\var{\la k{\la n{\la\elem\la \strtwo{nNNN_\ems k}}}}) (\la\varthree \writel\,\varthree)  k\,\enc{\ntostr n}\, \enc\elem\, \enc{\str}
\\ & \tob^{4} &
\enc{\ntostr n} N'N' (N_{\ems}\isub\strtwo{\enc\str}) k
\end{array}\]
where $N' \defeq N\isub\var{\la\varthree \writel\,\varthree}\isub{n}{\enc{\ntostr n}}\isub\strtwo{\enc\str}$.

Cases of $n$:
\begin{itemize}
\item $n=0$, and so $\ntostr n = \ems$: then  
\[\begin{array}{llllllll}
&&\enc{\ems} N'N' (N_{\ems}\isub\strtwo{\enc\str}) k 
\\ & = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) N'N' (N_{\ems}\isub\strtwo{\enc\str}) k 
\\ & \tob^{3} &
N_{\ems} \isub\strtwo{\enc\str} k
\\ & = &
\enc\str O_0 O_{1} O_{\ems} \cont
\end{array}\]
Cases of $\str$:
\begin{itemize}
\item $\str$ starts with $\elemblank$, that is, $\str = \elemblank\cons\strtwo$:
\[\begin{array}{llllllll}
\enc{\elemblank\cons\strtwo} O_0 O_{1} O_{\elemblank} O_{\ems} \cont
& = & 
(\la{\var_0}{\la{\var_1}{\la\var_{\elemblank}\la\vartwo\var_{\elemblank} \enc\strtwo}}) O_0 O_{1} O_{\elemblank} O_{\ems} \cont
\\ & \tobdet^{3} &
O_{\elemblank} \enc\strtwo \cont
\\ & = &
\end{array}\]

\item $\str$ starts with $1$, that is, $\str = 1\cons\strtwo$:
\[\begin{array}{llllllll}
\enc{0\cons\strtwo} O_0 O_{1} O_{\ems} \cont
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_{1} \enc\strtwo}}) O_0 O_{1} O_{\ems} \cont
\\ & \tobdet^{3} &
O_{1} \enc\strtwo \cont
\\ & = &
(\la\varthree\la y y\cods{1}) \enc\strtwo \cont
\\ & \tob^{2} &
\cont \cods{1} 
\\ & = & 
\cont (\cods{\writef\, \ems (1\cons\strtwo)})
\end{array}\]
\end{itemize}

\item \emph{Non-empty string} $n>0$ and so $\ntostr n = \elem \cons \strthree$: then  
\[\begin{array}{llllllll}
&&\enc{\ntostr n} N'N'(N_{\ems}\isub\strtwo{\enc\str}) k 
\\ & = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo \var_{\elem} \enc{\strthree}}}) N'N'(N_{\ems}\isub\strtwo{\enc\str}) k 
\\ & \tob^{3} &
N' \enc{\strthree} k
\\ & = &
(\la\varthree \strtwo MM M_\ems)\isub\var{\la\varthree \writel\,\varthree}\isub{n}{\enc{\ntostr n}}\isub\strtwo{\enc\str} \enc{\strthree} \cont 
\\ & \tob &
\enc\str M'M' M_\ems \cont
\end{array}\]
where $M' \defeq M\isub\var{\la\varthree \writel\,\varthree}\isub{n}{\enc{\ntostr n}}$. Cases of $\str$:

\begin{itemize}
\item $\str$ is empty:
\[\begin{array}{llllllll}
\enc\ems M'M' M_\ems \cont
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\vartwo}}) M'M' M_\ems \cont
\\ & \tobdet^{3} &
M_\ems \cont
\\ & = &
(\la y y\cods{0}) \cont
\\ & \tob &
\cont \cods{0} 
\\ & = & 
\cont (\cods{\writef\, \ntostr n \ems})
\end{array}\]

\item $\str$ is non-empty, that is, $\str = \elem'\cons\strtwo$:
\[\begin{array}{llllllll}
\enc{\elem'\cons\strtwo} M'M' M_\ems \cont
& = & 
(\la{\var_0}{\la{\var_1}{\la\vartwo\var_{\elem'} \enc\strtwo}}) M'M' M_\ems \cont
\\ & \tobdet^{3} &
M' \enc\strtwo \cont
\\ & = &
((\la u{\la\cont{\predl(\var\cont )n u}})\isub\var{\la\varthree \writel\,\varthree}\isub{n}{\enc{\ntostr n}}) \enc\strtwo \cont
\\ & = &
(\la u{\la\cont{\predl((\la\varthree \writel\,\varthree)\cont )\enc{\ntostr n} u}}) \enc\strtwo \cont
\\ & \tob^{2} &
\predl((\la\varthree \writel\,\varthree)\cont )\enc{\ntostr n} \enc\strtwo 
\\ (\reflemma{pred}) & \tobdet^{\bigo{\size{\ntostr n}}} &
(\la\varthree \writel\,\varthree)\cont \enc{\predf\, \ntostr n} \enc\strtwo
\\ & \tobdet &
\writel\, \cont \enc{\predf\,\ntostr n} \enc\strtwo
\\ & = &
\writel\, \cont \enc{\ntostr{ n-1}} \enc\strtwo
\\ (\ih) & \tobdet^{\bigo{(n-1)\cdot\log{(n-1)}}} &
\cont (\cods{\writef\, \ntostr{n-1} \strtwo})
\\
\\ & = & 
\cont (\cods{\writef\, \ntostr n \str})
\end{array}\]

The number of $\beta$ steps then is $\bigo{\size{\ntostr n}} + \bigo{(n-1)\cdot\log{(n-1)}} + k$ for a certain constant $k$. Since $\size{\ntostr n} = \bigo{\log n}$, we obtain that the number of steps is bound by $\bigo{n\cdot\log{n}}$, as required.
\end{itemize}



\end{itemize}
\end{proof}
